Differential Private Knowledge Transfer for Privacy-Preserving Cross-Domain Recommendation

Cross Domain Recommendation (CDR) has been popularly studied to alleviate the cold-start and data sparsity problem commonly existed in recommender systems. CDR models can improve the recommendation performance of a target domain by leveraging the data of other source domains. However, most existing CDR models assume information can directly 'transfer across the bridge', ignoring the privacy issues. To solve the privacy concern in CDR, in this paper, we propose a novel two stage based privacy-preserving CDR framework (PriCDR). In the first stage, we propose two methods, i.e., Johnson-Lindenstrauss Transform (JLT) based and Sparse-awareJLT (SJLT) based, to publish the rating matrix of the source domain using differential privacy. We theoretically analyze the privacy and utility of our proposed differential privacy based rating publishing methods. In the second stage, we propose a novel heterogeneous CDR model (HeteroCDR), which uses deep auto-encoder and deep neural network to model the published source rating matrix and target rating matrix respectively. To this end, PriCDR can not only protect the data privacy of the source domain, but also alleviate the data sparsity of the source domain. We conduct experiments on two benchmark datasets and the results demonstrate the effectiveness of our proposed PriCDR and HeteroCDR.

==> Privacy-Preserving CDR/sections/analysis.tex <==
\section{Analysis}\label{sec:ana}

In this section, we provide privacy and utility analysis of our proposed DP rating publishing algorithm (Algorithm~\ref{alg:dp_rating_pub}).  

% Privacy analysis 

%---------------------------------------------------------------------------------------------------------------------------------------------------
%
%									Privacy Analysis 						
%
%---------------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Privacy Analysis}
% In this section, we derive the privacy property of the two proposed random DP publishing algorithms, Algorithm~\ref{alg:dp_graph} and Algorithm~\ref{alg:dp_graph2}.
%
Differential Privacy~\cite{dwork2014algorithmic} is a rigorous mathematics definition to measure the difficulty for an adversary to identify the presence or absence of any individual in a data-set via leveraging the output of a random algorithm $\M$. 
%
A general way to analyze the privacy of a random algorithm $\M$ is to tail bound the privacy loss random variable, defined by the log of the division of the output distributions on neighboring data sets.  
%
Thus, to provide the privacy analysis of Algorithm~\ref{alg:dp_rating_pub}, we study how the output distribution changes by differ exactly one user-item rating $r_{ij}$ in the input rating matrix $\mathbf{R}$. 
%

We will first show the eigenvalue interlacing for rating matrix in Lemma~\ref{lem:interlace_2}. 
%
By the eigenvalue interlacing results, we will then present the upper and lower bounds for privacy loss in Lemma~\ref{lem:upper} and Lemma~\ref{lem:lower} respectively. 
%
After it, by combining with the k-fold Composition Theorem in Theorem~\ref{thm:k_fold_comp}, we will show that Algorithm~\ref{alg:dp_rating_pub} achieves $(\epsilon, \delta)$ in Theorem~\ref{thm:dp_graph}. 

\nosection{Eigenvalue interlacing for rating matrix}
%
Suppose we have two neighbouring rating matrices $\mathbf{R}$ and $\mathbf{R}'$ as defined in Definition~\ref{def:neigh_rating}. 
%
Without loss of generality, we assume a rating $r_{ij}$ is not in $\mathbf{R}$ but in $\mathbf{R'}$. 
%
With line 2 in Algorithm~\ref{alg:dp_rating_pub} performing on $\mathbf{R}$, we have that $r_{ij}$ is with the value $\frac{w}{m}$ in $\mathbf{R}$ and with the value $r_{ij} \leftarrow \frac{w}{m} + (1 - \frac{w}{m}) r_{ij}$ in $\mathbf{R}'$. 
Define the covariance matrix of $\mathbf{R}$ as 
$\mathbf{L} = \mathbf{R}^{\intercal} \mathbf{R}$. 
%
After using Algorithm~\ref{alg:dp_rating_pub},
the $(i,j)$ element in $\mathbf{L}$ becomes $l_{ij} + \left( 1 - \frac{w}{m} \right) \Delta l_{ij}$, where $\Delta l_{ij} = r_{ik}^{\intercal} r_{jk}$. 
%
Thus, we can derive the eigenvalue interlacing lemma (Lemma~\ref{lem:interlace_2}) by the eigenvalue interlacing for minors which we presented in Lemma 1 in Appendix. 

% \begin{lemma} 
% [Eigenvalue Interlacing for Minors] Let $\mathbf{A}$ be an $n \times n$ symmetric matrix with eigenvalues 
% $\lambda_1 \leq \lambda_2 \leq \cdots \lambda_n$, and $\mathbf{B}$ be any $(n-1) \times (n-1)$ principal minor sub-matrix of $\mathbf{A}$, with eigenvalues $\mu_1 \leq \mu_2 \leq \cdots \leq \mu_{n-1}.$ Then 
% $$
% \lambda_i \leq \mu_i \leq \lambda_{i+1}, \quad \forall 1 \leq i \leq n-1. 
% $$
% \label{lem:interlace_1}
% \end{lemma}

\begin{lemma} 
[Eigenvalue Interlacing for Rating Matrix]
Assume 
$ \mathbf{R}^{\intercal} = \mathbf{U \Sigma V^{\intercal}} and~ \mathbf{R'}^{\intercal} = \mathbf{ U' \Lambda V'^{\intercal}},$ with 
$\mathbf{\Sigma} = \rm{diag} \left( \begin{bmatrix} \sigma_1, \cdots, \sigma_{n-1}, \sigma_n \end{bmatrix}  \right)$ 
and 
$\mathbf{\Lambda} = \rm{diag} \left( \begin{bmatrix} \lambda_1, \cdots, \lambda_{n-1}, \lambda_n \end{bmatrix}  \right)$ 
be the singular values of~$\mathbf{R}$~and~$\mathbf{R'}$ respectively, we have   
$$
\forall i, \quad \sigma_i \leq \lambda_i \leq \sigma_{i+1}. 
$$
\label{lem:interlace_2}
\end{lemma}

\begin{proof}
\ccc{Proof. in appendix}
\end{proof}

%---------------------------------------------------------------------------------------------------------------------------------------------------
%
%						Johnson-Lindenstrauss Transform 
%
%---------------------------------------------------------------------------------------------------------------------------------------------------

\nosection{Analysis for user-level differential privacy?}
\ccc{rewrite this para.}
\nosection{Lower and upper bounds for privacy loss in one row}
%
To guarantee the privacy of Algorithm~\ref{alg:dp_graph} and Algorithm~\ref{alg:dp_graph2}, we analyze how the output distribution changes as exactly one value changes in the input rating matrix. 
% 
% We outline the proof of Algorithm~\ref{alg:dp_graph} as follows. 
%
Suppose $\mathbf{R}$ and $\mathbf{R'}$ are two neighbouring rating matrices as defined in Definition~\ref{def:neigh_rating}. 
%
As the privacy loss $L_{\M}^{\mathbf{R}, \mathbf{R'}}$ defined in Definition~\ref{def:privacy_loss}, we are interested in the difference of output distributions $\M(\mathbf{R})$ and $\M(\mathbf{R}')$. 
%
To do this, we first summarize Algorithm~\ref{alg:dp_graph} and Algorithm~\ref{alg:dp_graph2} as follows. 

\noindent\textit{Algorithm ~\ref{alg:dp_graph}.}
We summarize Algorithm~\ref{alg:dp_graph} as the following two operations on the input rating matrix $\mathbf{R}$, i.e., 
\begin{itemize}
    \item $\mathbf{R} \leftarrow \frac{w}{m}  \mathbf{I} + (1 - \frac{w}{m}) \mathbf{R}$, 
    \item $\mathbf{\tilde{R}} = \mathbf{M} \mathbf{R},$ with $\mathbf{M} \sim \GN(0, \mathbf{I}_{n_1' \times n_1})$, 
\end{itemize}
where $\mathbf{M}$ is constructed by concatenating $n'_1$ i.i.d. random Gaussian vectors $\mathbf{Y} \sim \GN(\mathbf{0}, \mathbf{I}_{n \times 1})$. 

%
In order to check the distribution between the output rating matrices $\mathbf{\tilde{R}}$ and $\mathbf{\tilde{R}'}$, we first compare the difference in Probability Density Function (PDF) of a single row in $\mathbf{\tilde{R}}$ and $\mathbf{\tilde{R}'}$, i.e., 
$\mathbf{R}^{\intercal} \mathbf{Y}$ and ${\mathbf{R}'}^{\intercal} \mathbf{Y}$.


% \huiwen{arrive the same intermediate results in Lemma 2 and Lemma 3}
\noindent\textit{Algorithm ~\ref{alg:dp_graph2}.}
Algorithm~\ref{alg:dp_graph2} is a modification of Algorithm~\ref{alg:dp_graph}. 
%
Specifically, in the step operation, the random transform is changed from a Gaussian orthogonal ensemble $\textbf{M}$ defined in Definition~\ref{def:jlt} to a sparse Johnson-Lindenstrauss transform, i.e., $\mathbf{PHD}$, defined in Definition~\ref{def:fjlt}, where $\mathbf{P}$ is a sparse Gaussian matrix, $\mathbf{H}$ is a Hadamard matrix and $\mathbf{D}$ is a random diagonal matrix. 
%
By construction, we have two good properties for Algorithm~\ref{alg:dp_graph2}. 
\begin{itemize}
    \item $\mathbf{D}$ and $\mathbf{U}$ are unitary, i.e., 
    $
    \mathbf{D}^{\intercal} \mathbf{D} = \mathbf{I}; \quad 
    \mathbf{U}^{\intercal} \mathbf{U} = \mathbf{I}, 
    $
    \item Rows in $\mathbf{P}$ are sub-Gaussian, 
\end{itemize}
%
where $\mathbf{P}$ is constructed by concatenating $n'_1$ i.i.d. sparse random Gaussian vectors $\mathbf{Y}$, where 
$$
\mathbf{Y}_i = 
\begin{cases}
0, \quad & \quad \text{with probability } 1-q; \\
\xi \sim \GN(0, q^{-1})& \quad \text{with probability } q. 
\end{cases}
$$


%
In order to check the distribution between $\mathbf{\tilde{R}}$ and $\mathbf{\tilde{R}}'$, for Algorithm~\ref{alg:dp_graph} and Algorithm~\ref{alg:dp_graph2}, we compare the difference in Probability Density Function (PDF) of a single row in $\mathbf{\tilde{R}}$ and $\mathbf{\tilde{R}'}$, i.e., 
$\mathbf{R}^{\intercal} \mathbf{Y}$ and ${\mathbf{R}'}^{\intercal} \mathbf{Y}$,  with $\mathbf{Y}$ denoting a Gaussian vector or sparse Gaussian vector.
%
%--------------------------------------------------%
%
%           User-level Differential Privacy 
%
%---------------------------------------------------%

In this section, we present the privacy loss of a single row in differential private published rating matrix $\mathbf{\tilde{R}},$ i.e., user-level differential privacy. The main result is described as follows. 

\begin{lemma}
Suppose $\mathbf{R}$ and $\mathbf{R}'$ are two neighbouring rating matrix as defined in Definition~\ref{def:neigh_rating}. 
%
$\mathbf{Y}$ is Gaussian random vectors defined before. 
%

\end{lemma}


% we focus on the privacy property by comparing the distributions $\mathbf{R}^{\intercal} \mathbf{Y}$ and $\mathbf{R}'^{\intercal} \mathbf{Y}.$ \ccc{where is $\mathbf{\tilde{R}}'$ for algo. 2?}
%
% Through previous analysis \ccc{where?}, one can explore the difference of distribution on one row of the output matrices, i.e., $\mathbf{R}^{\intercal} \mathbf{Y}$ and $\mathbf{R}'^{\intercal} \mathbf{Y}$, with $\mathbf{Y}$ denoting a Gaussian vector or sparse Gaussian vector.
%
% With the similar deduction, we arrive the same lower and upper bound of the difference between $\pdf_{\mathbf{R}^{\intercal} \mathbf{Y}}$ and $\pdf_{\mathbf{R}'^{\intercal} \mathbf{Y}}$ for Algorithm~\ref{alg:dp_graph} and Algorithm~\ref{alg:dp_graph2}, and we summarize them in Lemma~\ref{lem:lower} and Lemma~\ref{lem:upper} respectively. 

% \begin{lemma} [Lower Bound] \label{lem:lower}
% Set $\epsilon_0 = \frac{\epsilon}{\sqrt{4 n_1' \ln(2/\delta)}}$, $ \delta_0 = \frac{\delta}{2 n_1'}$, and denote $S = \{ x: \pdf_{\mathbf{R}^{\intercal} \mathbf{Y}} (x) \geq e^{-\epsilon_0}  \pdf_{\mathbf{R}^{\intercal} \mathbf{Y}} (x) \}$ with $\mathbf{Y}_{n_1 \times 1}$ a Gaussian random vector or a sparse Gaussian random vector, 
% we have
% \begin{equation} \label{eqn:lower}
% P (S) \geq 1 - \delta_0. 
% \end{equation}
% \end{lemma}

% \begin{lemma} [Upper Bound] \label{lem:upper}
% Set $\epsilon_0 = \frac{\epsilon}{\sqrt{4 n_1' \ln(2/\delta)}}$, $ \delta_0 = \frac{\delta}{2 n_1'}$, 
% %$\mathbf{Y}$ is a random vector of size $n \times 1$ with every element is a normal random variable, i.e., $\mathbf{Y} \sim \GN(\mathbf{0}, \mathbf{I}_{n \times 1})$
% with $\mathbf{Y}_{n_1 \times 1}$ a Gaussian random vector or a sparse Gaussian random vector, 
% we have
% \begin{equation}\label{eqn:upper}
% \forall x, \pdf_{\mathbf{R}^{\intercal} \mathbf{Y}} (x) \leq e^{\epsilon_0} \pdf_{{\mathbf{R}'}^{\intercal} \mathbf{Y}} (x).
% \end{equation}
% \end{lemma}


% The rating matrix and the covariance matrix shares the same spectrum property as shown in Lemma~\ref{lem:interlace_2}. It is equivalent to compare the distributions of covariance matrices $\M(\mathbf{L})$ and $\M(\mathbf{L}')$. 
% %
% Under Algorithm~\ref{alg:dp_graph}, the output covariance matrix is to 
% $\mathbf{\tilde{L}}= \frac{1}{n_1'} \mathbf{R}^{\intercal} \mathbf{M}^{\intercal} \mathbf{M} \mathbf{R} = \mathbf{O}^{\intercal} \mathbf{O}$ and 
% $\mathbf{\tilde{L}'} = \frac{1}{n_1'} \mathbf{R}'^{\intercal} \mathbf{M}^{\intercal} \mathbf{M} \mathbf{R}' = \mathbf{O}'^{\intercal} \mathbf{O}'$ respectively, 
% with $M \sim \GN(\mathbf{0}, \mathbf{I}_{d' \times n})$ a Gaussian orthogonal ensemble (GOE) as defined in Definition~\ref{def:jlt}. 
% % 
% We concate $\mathbf{O}$ by $k$ i.i.d. random vector $Y \sim \GN(\mathbf{0}, \mathbf{I}_{n \times 1})$. 
% %
% In order to check the distribution between the output covariance matrices $\mathbf{\tilde{L}}$ and $\mathbf{\tilde{L}'}$, we first compare the difference in probability density function of $\mathbf{R}{\intercal} Y$ and $\mathbf{R}^{\intercal} Y$.
%
% In the following lemma, we prove the upper bound of the difference between $\pdf_{\mathbf{R}^{\intercal} \mathbf{Y}}$ and $\pdf_{{\mathbf{R}'}^{\intercal} \mathbf{Y}}. $


% \begin{lemma} \label{lem:upper}
% Set $\epsilon_0 = \frac{\epsilon}{\sqrt{4 r \ln(2/\delta)}}, \delta_0 = \frac{\delta}{2r}.$
% $\mathbf{Y}$ is a random vector of size $n \times 1$ with every element is a normal random variable, i.e. $\mathbf{Y} \sim \GN(\mathbf{0}, \mathbf{I}_{n \times 1})$
% Then 
% \begin{equation}\label{eqn:upper}
% \forall x, \pdf_{\mathbf{R}^{\intercal} \mathbf{Y}} (x) \leq e^{\epsilon_0} \pdf_{{\mathbf{R}'}^{\intercal} \mathbf{Y}} (x).
% \end{equation}

% \end{lemma}

% Then we comes to the lower bound of the difference between two distributions $\pdf_{\mathbf{R}^{\intercal} \mathbf{Y}}$ and $\pdf_{{\mathbf{R}'}^{\intercal} \mathbf{Y}}. $


% \begin{lemma} \label{lem:lower}
% Set $\epsilon_0 = \frac{\epsilon}{\sqrt{4 r \ln(2/\delta)}}, \delta_0 = \frac{\delta}{2r}.$
% And denote $S = \{ x: \pdf_{\mathbf{R}^{\intercal}_G \mathbf{Y}} (x) \geq e^{-\epsilon_0}  \pdf_{\mathbf{R}^{\intercal}_{G'} \mathbf{Y}} (x) \}$
% \begin{equation} \label{eqn:lower}
% P (S) \geq 1 - \delta_0
% \end{equation}
% \end{lemma}



%---------------------------------------------------------------------------------------------------------------------------------------------------
%
%						Fast Johnson-Lindenstrauss Transform 
%
%---------------------------------------------------------------------------------------------------------------------------------------------------
%
% To guarantee privacy of Algorithm~\ref{alg:dp_graph2}, we are interested in the distributions of output covariance matrices
% $\mathbf{\tilde{L}}$ and $\mathbf{\tilde{L}'}$ on the two neighboring rating values $\mathbf{R}$ and $\mathbf{R}'.$
% %
% Under Algorithm~\ref{alg:dp_graph2}, the output covariance matrix is
% $\mathbf{\tilde{L}} = \frac{1}{d'} \mathbf{R}^{\intercal} (\mathbf{PHD})^{\intercal} \mathbf{PHD} \mathbf{R} = \frac{1}{d'} \mathbf{R}^{\intercal} \mathbf{P}^{\intercal} \mathbf{P} \mathbf{R}$ and 
% $\mathbf{\tilde{L}'} = \frac{1}{d'} \mathbf{R'}^{\intercal} (\mathbf{PHD})^{\intercal} \mathbf{PHD} \mathbf{R'} = \frac{1}{d'} 
% \mathbf{R'}^{\intercal} \mathbf{P}^{\intercal} \mathbf{P} \mathbf{R'}$ respectively, 
% with $\mathbf{P}$ is a sparse Gaussian matrix, $\mathbf{H}$ is a Hadamard matrix and $\mathbf{D}$ is a diagonal matrix as defined in Algorithm~\ref{alg:dp_graph2}. 
% By construction, $\mathbf{D}$ and $\mathbf{U}$ are unitary, i.e., 
% $$
% \mathbf{D}^{\intercal} \mathbf{D} = \mathbf{I}; \quad 
% \mathbf{U}^{\intercal} \mathbf{U} = \mathbf{I}. 
% $$
% %
% We construct $\mathbf{P}$ by $k$ i.i.d. sparse random Gaussian vector $\mathbf{Y}$. 
% %
% In order to check the distribution between $\mathbf{\tilde{L}}$ and $\mathbf{\tilde{L}}'$, we focus on the privacy property by comparing the distributions $\mathbf{R}^{\intercal} \mathbf{Y}$ and $\mathbf{R}'^{\intercal} Y.$
% %
% With similar deduction in previous section, we prove the upper bound of the difference between $\pdf_{\mathbf{R}^{\intercal} \mathbf{Y}}$ and $\pdf_{\mathbf{R}'^{\intercal} \mathbf{Y}}. $


% \begin{lemma} \label{lem:upper2}
% Set $\epsilon_0 = \frac{\epsilon}{\sqrt{4 r \ln(2/\delta)}}, \delta_0 = \frac{\delta}{2r}.$
% Then 
% \begin{equation}\label{eqn:upper2}
% \forall x, \pdf_{\mathbf{R}^{\intercal}_G \mathbf{Y}} (x) \leq e^{\epsilon_0} \pdf_{\mathbf{R}^{\intercal}_{G'} \mathbf{Y}} (x).
% \end{equation}
% \end{lemma}

% Then we get the lower bound of the difference between two distributions $\pdf_{\mathbf{R}^{\intercal}_G \mathbf{Y}}$ and $\pdf_{\mathbf{R}^{\intercal}_{G'} \mathbf{Y}}$. 
% \ccc{cannot follow}
% \huiwen{try to see the difference between the two distributions, pdf -- probability density function.}

% \begin{lemma} \label{lem:lower2}
% Set $\epsilon_0 = \frac{\epsilon}{\sqrt{4 r \ln(2/\delta)}}, \delta_0 = \frac{\delta}{2r}.$
% And denote $S = \{ x: \pdf_{\mathbf{R}^{\intercal}_G \mathbf{Y}} (x) \geq e^{-\epsilon_0}  \pdf_{\mathbf{R}^{\intercal}_{G'} \mathbf{Y}} (x) \}$
% \begin{equation} \label{eqn:lower2}
% P (S) \geq 1 - \delta_0
% \end{equation}
% \end{lemma}



%---------------------------------------------------------------------------------------------------------------------------------------------------
\nosection{Analysis for rating-level differential privacy?}
\ccc{rewrite this para.}
\nosection{Differential privacy rating publishing algorithms}
By previous lower and upper bounds, we compare the distribution difference of a single row in output rating matrix $\mathbf{\tilde{R}}$ and $\mathbf{\tilde{R}}'$. To analyze the difference of two whole rating matrices $\mathbf{\tilde{R}}$ and $\mathbf{\tilde{R}}'$, we utilize the following composition theorem presented in Theorem~\ref{thm:k_fold_comp}. 

\begin{theorem} [Composition Theorem \cite{dwork2010boosting}]
For every $\epsilon >0, \delta, \delta' >0$, and $k \mathbb{N},$ the class of $(\epsilon, \delta)-$differential private mechanisms is 
$(\epsilon', k \delta + \delta')-$differentially private under $k-$fold adaptive composition, for 
$
\epsilon' = \sqrt{2k \ln (1/\delta')} \epsilon + k \epsilon \epsilon_0
$,
where $\epsilon_0 = e^{\epsilon} -1.$
\label{thm:k_fold_comp}
\end{theorem}

With the privacy guarantee of one row in $\mathbf{R}$ and composition theorem, we present differential privacy with respect to rating value of Algorithm~\ref{alg:dp_graph} and Algorithm~\ref{alg:dp_graph2}.

\begin{theorem}[Rating matrix differential privacy] %\cite{blocki2012johnson}
%of Algorithm~\ref{alg:dp_graph}]
Algorithm~\ref{alg:dp_graph} and Algorithm~\ref{alg:dp_graph2} preserve $(\epsilon, \delta)-$differential privacy with respect to a single rating value changing in $\mathbf{R}$. 
\label{thm:dp_graph}
\end{theorem}

\begin{proof}
\ccc{add proof description?}
\end{proof}

%---------------------------------------------------------------------------------------------------------------------------------------------------
%
%						Utility Analysis 
%
%---------------------------------------------------------------------------------------------------------------------------------------------------

\subsection{Utility Analysis}
\label{sec:utility_ana}

In this section, we present the utility analysis of differential private rating matrix publishing mechanism, Algorithm~\ref{alg:dp_graph} and Algorithm~\ref{alg:dp_graph2} with concentration results of JLT and SJTL. 

\begin{theorem}
[Concentration of JLT~\cite{upadhyay2013random} and SJLT~\cite{ailon2009fast}]
For any $\eta \in (0, 1/2)$ and $M$ be a $n_1' \times n_1$ random matrix, as defined in Definition~\ref{def:jlt} or Definition~\ref{def:fjlt}. 
For $\forall \mathbf{x} \in \mathbb{R}^n,$ let $S =\{ \x:  (1- \eta) \| \x \|^2 \leq \frac{1}{n_1'} \| \mathbf{M} \x \|^2 \leq (1 + \eta) \| \x \|^2 \}$, we have
$$
P\left[ S \right] \geq 1- 2 \exp(- \eta^2 n_1'/8). 
$$
\label{thm:con_jlt}
\end{theorem}

% It is easy to check $\mathbf{HD}$ is $\ell_2-$norm preserving. $\mathbf{P}$ is a sparsity version of $M$, then we have the concentration results of 
% $\mathbf{PHD}$, i.e., 

% \begin{theorem}[Concentration of SJLT~\cite{ailon2009fast}]
% Suppose the same assumptions as described in Theorem~\ref{thm:con_jlt}.
% Let $\mathbf{P}, \mathbf{H}, \mathbf{D}$ be random matrices as defined in Definition~\ref{def:fjlt}. 
% Let $S = \{\x: (1- \eta) \| \x \|^2 \leq \frac{1}{n_1'} \| \mathbf{PHD} \x \|^2 \leq (1 + \eta) \| \x \|^2 \}$, we have 
% $$
% \mathbf{P} \left[ S  \right] \geq 1 -2 \exp (- \eta^2 n_1'/8). 
% $$
% \label{thm:con_fjlt}
% \end{theorem}

Following the concentration results of Johnson-Lindenstrauss (Theorem~\ref{thm:con_jlt} and Theorem~\ref{thm:con_fjlt}), 
%and the algorithm approximating $\Phi_G$ (Algorithm~\ref{alg:phi_approx}),
we have the utility guarantees of Algorithm~\ref{alg:dp_graph} and Algorithm~\ref{alg:dp_graph2}. For details of proof, please refer to ~\cite{blocki2012johnson}.
%
Furthermore, 
with random transform used in Algorithm~\ref{alg:dp_graph} and Algorithm ~\ref{alg:dp_graph2}, we have a good approximation of the original rating matrix $\mathbf{R}$ with a large probability, as is shown in Theorem~\ref{thm:dp_approx}. 


\begin{theorem}[Approximation Property~\cite{blocki2012johnson}]
For every $\eta, \mu > 0$, $\tau = O \left(s \frac{\sqrt{\ln(1/\delta) \ln(1/\mu)}}{\epsilon}  \left( \ln(1/\delta) + \ln(\ln(1/\mu)/ \eta^2) \right)\right)$, and a nonempty $S$ of size $s$, Algorithm~\ref{alg:dp_graph} and Algorithm~\ref{alg:dp_graph2} give a $(\eta, \tau, \mu)-$approximation for rating matrix $\mathbf{R}$.
~\label{thm:dp_approx}
\end{theorem}



















==> Privacy-Preserving CDR/sections/analysis1.tex <==
\section{Analysis}\label{sec:ana}

% In this section, we analyze the privacy and utility of Algorithm~\ref{alg:dp_rating_pub}.  


%---------------------------------------------------------------------------------------------------------------------------------------------------
%
%									Privacy Analysis 						
%
%---------------------------------------------------------------------------------------------------------------------------------------------------

\subsection{Privacy Analysis}

% Differential Privacy~\cite{dwork2014algorithmic} is a rigorous mathematics definition to measure the difficulty for an adversary to identify the presence or absence of any individual in a data-set via leveraging the output of a random algorithm $\M$. 
% %
% A general way to analyze the privacy of a random algorithm $\M$ is to tail bound the privacy loss define in Definition~\ref{def:privacy_loss}. 
%
To analyze the privacy of Algorithm~\ref{alg:dp_rating_pub}, we study how the output distribution changes for neighbouring rating matrices and how to achieve both user-level DP and rating matrix DP. %in  Definition~\ref{def:neigh_user_rating} and ~\ref{def:rating_dp}. 
%
%---------------------------------------------------------------------------------------------------------------------------------------------------
%
%									sub1: User-level Differential Privacy 				
%
%---------------------------------------------------------------------------------------------------------------------------------------------------

\nosection{User-level differential privacy}
We first present the user-level differential privacy, i.e., privacy loss for a single row in differential private published rating matrix. 
%
% Inspired by the result that JLT preserves DP~\cite{blocki2012johnson}, we further study the privacy-preserving property of SJLT~\cite{ailon2009fast}. 
%
In Theorem~\ref{thm:user_dp}, we show that both JLT and SJLT achieve user-level DP. 
%
% For details, check appendix \ref{sec:append_user_dp}. 

\begin{theorem} [User-level Differential Privacy]
\label{thm:user_dp}
%
Suppose $\mathbf{R}$ and $\mathbf{R'}$ are two neighbouring rating matrices as defined in Definition~\ref{def:neigh_rating}. 
%
Let $\mathbf{Y} \sim \mathbf{N}(0, 1)$ be a random vector. 
%
Define the two distributions of $\mathbf{R^{\intercal}Y}$ and $\mathbf{R'^{\intercal}Y}$ respectively as 
\begin{eqnarray*}
\pdf_{\mathbf{R}^{\intercal} \mathbf{Y}} & = & \frac{1}{\sqrt{ (2 \pi)^{n_1} \rm{det} (\mathbf{R}^{\intercal} \mathbf{R})}}
\exp \left( - \frac{1}{2} \mathbf{x}^{\intercal} \left( \mathbf{R^{\intercal} R} \right)^{-1} \mathbf{x} \right), \\
\pdf_{\mathbf{R'}^{\intercal} \mathbf{Y}} & = & \frac{1}{\sqrt{ (2 \pi)^{n_1} \rm{det} (\mathbf{R'}^{\intercal} \mathbf{R'})}}
\exp \left( - \frac{1}{2} \mathbf{x}^{\intercal} \left( \mathbf{R'^{\intercal} R'} \right)^{-1} \mathbf{x} \right). \\
\end{eqnarray*}
%
Fix $\epsilon_0 = \frac{\epsilon}{\sqrt{4r \ln(2/\delta)}}$ and $\delta_0 = \frac{\delta}{2r}$, and  
%
denote $\mathcal{S} = \{ x: e^{- \epsilon_0} \pdf_{\mathbf{R'^{\intercal} Y}} (x) \leq \pdf_{\mathbf{R^{\intercal} Y}}(x) \leq e^{\epsilon_0} 
\pdf_{\mathbf{R'^{\intercal} Y}} (x) \}$, 
%
then we have 
$\Pr[\mathcal{S}] \geq 1 - \delta_0$. 
%
Thus Algorithm~\ref{alg:dp_rating_pub} preserves $(\epsilon_0, \delta_0)-$DP for each row in the published rating matrix. 
\end{theorem}

\begin{proof}
We present its proof in Appendix~\ref{sec:append_user_dp}.
\end{proof}
 
%
%The only difference between JLT and SJLT is the method to generate the random matrix. 
%
% JLT is generated under Gaussian distribution, see Definition~\ref{def:jlt} while SJLT is generated by the product of the sub-Gaussian matrix $P$, the normalized Hadamard random matrix, and a diagonal random matrix. 
%

%---------------------------------------------------------------------------------------------------------------------------------------------------
%
%									sub2: Rating Matrix Differential Privacy 					
%
%---------------------------------------------------------------------------------------------------------------------------------------------------


\nosection{Rating matrix differential privacy}
Based on user-level privacy guarantees (Theorem~\ref{thm:user_dp}) and the k-fold composition theorem (Theorem~\ref{thm:k_fold_comp} in Appendix), we present differential privacy with respect to rating value of Algorithm~\ref{alg:dp_rating_pub}.

\begin{theorem}[Rating Matrix Differential Privacy] %\cite{blocki2012johnson}
%of Algorithm~\ref{alg:dp_graph}]
Algorithm~\ref{alg:dp_rating_pub} preserves $(\epsilon, \delta)-$differential privacy with respect to a single rating value changing in $\mathbf{R}$. 
\label{thm:dp_graph}
\end{theorem}

\begin{proof}
We present its proof in Appendix~\ref{sec:rating_dp_append}.
\end{proof}

By presenting privacy guarantees for user-level and rating matrix, we show our algorithm achieves \textbf{G1}: \textit{Privacy-preserving}. 
%---------------------------------------------------------------------------------------------------------------------------------------------------
%
%									Utility Analysis 						
%
%---------------------------------------------------------------------------------------------------------------------------------------------------

\subsection{Utility Analysis}
\label{sec:utility_ana}

We analyze the utility of Algorithm~\ref{alg:dp_rating_pub} from a probabilistic perspective. 
%
First, we show that the expectation of the perturbed published rating matrix on the low-dimensional subspace approximates the input rating matrix on the high-dimensional original space, with a bias determined by privacy parameters (Theorem~\ref{prop:mean_approx}). 
%
Based on the expectation approximation, we show Algorithm~\ref{alg:dp_rating_pub} achieves \textit{Restricted isometry property}, i.e., the output rating matrix concentrates around the mean approximation with a large probability determined by privacy parameters (Theorem~\ref{thm:RIP}). 

%\huiwen{move to appendix}
% \begin{theorem}\label{thm:con_jlt}
% [Concentration of JLT~\cite{upadhyay2013random} and SJLT~\cite{ailon2009fast}]
% For any $\eta \in (0, 1/2)$ and $M$ be a $n_1' \times n_1$ random matrix, as defined in Definition~\ref{def:jlt} or Definition~\ref{def:fjlt}. 
% For $\forall \mathbf{x} \in \mathbb{R}^n,$ let $S =\{ \x:  (1- \eta) \| \x \|^2 \leq \frac{1}{n_1'} \| \mathbf{M} \x \|^2 \leq (1 + \eta) \| \x \|^2 \}$, we have
% $$
% \Pr \left[ S \right] \geq 1- 2 \exp(- \eta^2 n_1'/8). 
% $$
% \label{thm:con_concen}
% \end{theorem}

% Following the concentration results (Theorem~\ref{thm:con_jlt}), 
% we prove the approximation property of original rating matrix in nuclear norm in Proposition~\ref{prop:mean_approx} and restricted isometry property in Theorem~\ref{thm:RIP}, which demonstrate the utility guarantee of Algorithm~\ref{alg:dp_rating_pub}.
% %and the algorithm approximating $\Phi_G$ (Algorithm~\ref{alg:phi_approx}),
% we have the utility guarantee of Algorithm~\ref{alg:dp_rating_pub}. \ccc{where?}
% %
% For details of proof, please refer to ~\cite{blocki2012johnson}.
% %
% Furthermore, 
% with random transform used in Algorithm~\ref{alg:dp_rating_pub}, we have a good approximation of the original rating matrix $\mathbf{R}$ with a large probability, as is shown in Proposition~\ref{prop:mean_approx} and Theorem~\ref{thm:RIP}.


%---------------------------------------------------------------------------------------------------------------------------------------------------
%
%									sub1: Unbiased Mean 				
%
%---------------------------------------------------------------------------------------------------------------------------------------------------
\nosection{Expectation approximation}
%
We first present the approximation effect of the published rating matrix to original one, which is the foundation of \text{restricted isometry property}. 
%
\begin{proposition}
\label{prop:mean_approx}
Let $\mathbf{R}$ and $\mathbf{\tilde{R}}$ be the input and output rating matrix of Algorithm~\ref{alg:dp_rating_pub}, respectively. 
%
Then, the mean squared error of the input and output covariance matrices are 
$$
\E \| \mathbf{R^{\intercal} R} - \mathbf{\tilde{R}^{\intercal} \tilde{R}} \|_2^2 \leq w^2 m 
= 16 n_1'^2 \ln(2/\delta) \ln^2(4 n_1'/\delta) / \epsilon^2 m, 
 $$
where 
$n_1' $ is the dimension of the reduced item space,  
$m $ is the number of user, and 
$(\epsilon, \delta)$ are privacy parameters. 
\end{proposition}
%
\begin{proof}
We present its proof in Appendix~\ref{sub:mean_append}.
\end{proof}
% We present the proof of Proposition~\ref{prop:mean_approx} in Appendix~\ref{sub:mean_append}. 

%---------------------------------------------------------------------------------------------------------------------------------------------------
%
%									sub2: Concentration Results 				
%
%---------------------------------------------------------------------------------------------------------------------------------------------------
\nosection{Restricted isometry property}
We then come to the main results--- Algorithm~\ref{alg:dp_rating_pub} has \textit{Restricted isometry property}. 

\begin{theorem}
[Restricted Isometry Property]
\label{thm:RIP}
Let $\mathbf{R}$ and $\mathbf{\tilde{R}}$ be the input and output rating matrix of Algorithm~\ref{alg:dp_rating_pub}, respectively. 
%
Then 
\begin{align*}
& \Pr \left[  \left( 1 - \gamma \right)  \left(  \| \mathbf{R}   \|_F^2 + w^2 m  \right)   \leq \| \mathbf{\tilde{R} \|_F^2 }
\leq \left( 1 + \gamma \right)  \left(  \| \mathbf{R}   \|_F^2 + w^2 m  \right)  \right] \\
 & \leq  1 - 2 n_1'^{-2m},
\end{align*}
where $n_1'$  is the dimension of reduced item space,
$m$ is the number of user,
and $\gamma = O(\sqrt{\frac{\log m }{n_1'}}). $
\end{theorem}
%

\begin{proof}
We present its proof in Appendix~\ref{sub:RIP_append}.
\end{proof}
% We present the proof of Theorem~\ref{thm:RIP} in \ref{sub:RIP_append}.

By the concentration results, we see that the larger subspace dimension $n_1'$, the larger probability
 $  \| \mathbf{\tilde{R}} \|_F^2 $ approximated $  \| \mathbf{R} \|_F^2  + w^2 m$ with a distance of $\epsilon$, which verifies the conclusion. 


%---------------------------------------------------------------------------------------------------------------------------------------------------
%
%									SJLT 					
%
%---------------------------------------------------------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------
%
%                           Goal (3)
%
%--------------------------------------------------------------------------
\nosection{Improvement of SJLT}
Furthermore, we explain how SJLT improves JLT from the perspective of preconditioning. 
%
Applying SJLT on a vector $\mathbf{x}$, we have $\mathbf{PHDx}$. 
%
%Before applying a sparse random sub-Gaussian transform $\mathbf{P}$, we have $\mathbf{HD}$ serves as precondioner. 
%
Since $\mathbf{H}$ and $\mathbf{D}$ are unitary,  $\mathbf{HD}$ preserves $\ell_2-$norm, i.e., $\| \mathbf{HDx} \|_2 = \| \mathbf{x}\|_2$. 
%
\begin{lemma}[Randomized Hardmard transform~\cite{ailon2009fast}]
Let $\mathbf{H}$ and $\mathbf{D}$ be defined in Definition~\ref{def:fjlt}. For any set $V$ of $m$ vectors in $\mathbf{R}^{n_1}$, with probability at least $1 - 1/20$, 
$$
\max_{x \in V} \| \mathbf{HDx} \|_{\infty} \leq \left( \frac{2 \ln(40 m n_1)}{n_1} \right)^{1/2} \| \mathbf{x} \|_2. 
$$
\label{lem:rhd}
\end{lemma}
%
% We present the proof of Lemma~\ref{lem:rhd} in Appendix~\ref{sec:rhd_append}. 

\begin{proof}
We present its proof in Appendix~\ref{sec:rhd_append}.
\end{proof}

By Lemma~\ref{lem:rhd}, we observe that the preconditioner $\mathbf{HD}$ reduces the $\ell_{\infty}-$norm of $\mathbf{x}$. 
%
With the same $\ell_2$-norm and reduced $\ell_{\infty}-$norm, the energy of vector $\mathbf{x}$ is spread out. 
%
That is, the preconditioner $\mathbf{HD}$ smoothes out the sparse vector $\mathbf{x}$ and improves the utility of sparse sub-Gaussian transform $\mathbf{P}$. 
%
To this end, our algorithm achieves \textbf{G2} (restricted isometry property) and \textbf{G3} (sparse-aware). 

%%-----------------------------------------------------------------------
%%          benefits of sparsity 
%%-----------------------------------------------------------------------
% \nosection{Sparsity benefits of SJLT}
% Recall the random matrix generation in SJLT we have $\mathbf{M} = \mathbf{PHD}$ in Definition~\ref{def:fjlt}. In the previous section, we outline the benefits of randomized Hadamard transform $\mathbf{HD}$ from the preconditioning perspective. Now we consider the benefits of the sparse random matrix $\mathbf{P}$. 
% %
% Increasing the sparsity in sparse random matrix $P$ improves the computation efficiency in matrix multiplication. The more zero elements, the fewer element-wise productions need to be computed. The complexity of sparse matrix multiplication reduces from $O(m n n_1)$ to $O(\rm{nnz}(\mathbf{P}))$, where $\rm{nnz}(\mathbf{P})$ denotes the number of non-zero elements in matrix $\mathbf{P}$. 
% %
% Existing works discuss the lower bound for sparsity parameter such that the sparse random transform grasps enough knowledge from the input data matrix~\cite{li2006very,drineas2011faster}
% %
% Moreover, we explain that the sparsity of sub-Gaussian transform $\mathbf{P}$ serves as an implicit regularization, which further improves the performance of the overall algorithm. 
% %
% For easy to understand, we take the example of linear regression. The deep learning models follow the same. 
% %
% The loss function of a linear regression model is 
% $$
% \mathcal{L} (\mathbf{w}, \mathbf{x}) =  \| \mathbf{y} - \left(  \langle \mathbf{w}, \mathbf{x} \rangle + \mathbf{b}  \right)  \|_2,
% $$
% where $\mathbf{w}, \mathbf{b}$ denotes the parameters of model, 
% $\mathbf{x}$ denotes the data, 
% and $\mathbf{y}$ denotes the label.
% Consider a sparse random matrix $\mathbf{P}$ operating on $x$, we have 
% \begin{align*}
% \mathcal{L} (\mathbf{w}, \mathbf{P x}) &= \| \mathbf{y} - \left(  \langle \mathbf{w}, \mathbf{P x} \rangle + \mathbf{b}  \right)  \|_2 \\
% & = \| \mathbf{y} - \left(  \langle \mathbf{P^{\intercal} w}, \mathbf{x} \rangle + \mathbf{b}  \right)  \|_2 \\
% \end{align*}
% The minimization problem becomes 
% \begin{align*}
% \min \mathcal{L} (\mathbf{w}, \mathbf{P x})  & = \min \mathcal{L} (\mathbf{P^{\intercal} w}, x) \\
% & = \min_{\mathbf{w_1 = P w}} \mathcal{L} (\mathbf{w_1}, \mathbf{x}) \\
% & =  \min_{\mathbf{w}} \left( \mathcal{L} (\mathbf{w_1}, \mathbf{x}) + \lambda \|\mathbf{P^{\intercal} w} - \mathbf{w _1} \| \right), 
% \end{align*}
% Thus, the sparse random matrix $\mathbf{P}$ exerts an implicit regularization on the learned parameters $\mathbf{w}$, which eliminates the overfitting problem and improves accuracy. 

==> Privacy-Preserving CDR/sections/conclusion.tex <==
\section{Conclusion}
In this paper, we aim to solve the privacy issue in existing Cross Domain Recommendation (CDR) models. 
%
For this, we propose a novel two stage based privacy-preserving CDR framework, namely \modelname. 
%
In \textit{stage one}, the source domain privately publishes its user-item ratings to the target domain, and we propose two methods, i.e., Johnson-Lindenstrauss Transform (JLT) based and Sparse-aware JLT (SJLT) based, for it.  
%
We theoretically analyze the privacy and utility of our proposed differential privacy based rating publishing methods. 
%
In \textit{stage two}, the target domain builds a CDR model based on its raw data and the published data of the source domain, and we propose a novel heterogeneous CDR model (\cdrmodel) for it. 
%
We empirically study the effectiveness of our proposed \modelname~and \cdrmodel~on two benchmark datasets and the comprehensive experimental results show their effectiveness. 
%


==> Privacy-Preserving CDR/sections/experiment.tex <==
\section{Experiments and Analysis}
\label{sec:experi}

In this section, we conduct experiments on two real-world datasets to answer the following research questions. 
%
\textbf{RQ1}: How can our model outperform the state-of-the-art recommendation model that is trained using the data of the target domain only?
%
\textbf{RQ2}: What is the performance of our model compared with the state-of-the-art CDR models that are trained using both the plaintext source and target datasets? 
%
\textbf{RQ3}: Is our proposed CDR model (\cdrmodel) effective for the heterogeneous user-item rating data in the source and target domains?
%
\textbf{RQ4}: How do the parameters of JLT and SJLT (mainly $\epsilon$, $n$, and $sp$) in stage 1 affect our model performance?
%
\textbf{RQ5}: Will different data sparsity in the source domain affect the performance of JLT and SJLT? 
%
% \begin{itemize}[leftmargin=*] \setlength{\itemsep}{-\itemsep}
% \item \textbf{RQ1}: How can our model outperform the state-of-the-art recommendation model that is trained using the data of the target domain only?

% \item \textbf{RQ2}: What is the performance of our model compared with the state-of-the-art CDR models that are trained using both the plaintext source and target datasets? 


% \item \textbf{RQ3}: Is our proposed CDR model (\cdrmodel) effective for the heterogeneous user-item rating data in the source and target domains?

% \item \textbf{RQ4}: How do the parameters of JLT and SJLT (mainly $\epsilon$, $n$, and $sp$) in stage 1 affect our model performance?

% \item \textbf{RQ5}: Will different data sparsity in the source domain affect the performance of JLT and SJLT? 

% \end{itemize}

\subsection{Experimental Setup} 

\nosection{Datasets} 
We choose two real-world datasets, i.e., Amazon and Douban. 
%
The \textbf{Amazon} dataset \cite{amazon,catn} has three domains, i.e., Movies and TV (Movie), Books (Book), and CD Vinyl (Music). 
%
The \textbf{Douban} dataset \cite{zhu2019dtcdr,zhu2021unified} also has three domains, i.e., Book, Music, and Movie. 
%
Since the user-item interaction ratings in both datasets range from 0 to 5, we binarize them by taking the ratings that are higher or equal to 3 as positive and others as negative, following \cite{hu2018conet}. 
%
We also filter the users and items with less than 5 interactions. 
%
For simplification, we only choose the user-item interactions of the common users across domains. 
%
The detailed statistics of these datasets after pre-process are shown in Appendix \ref{sec:app:data}.


\nosection{Comparison methods} 
To validate the performance of our proposed model, 
%
we compare \modelname~and its variants (\textbf{PriCDR-SYM}, \textbf{PriCDR-J}, and \textbf{PriCDR-S}) with both the famous single domain recommendation methods (\textbf{BPR}, \textbf{NeuMF}, and \textbf{DMF}) and the state-of-the-art CDR methods (\textbf{CoNet}, \textbf{DDTCDR}, \textbf{DARec}, and \textbf{ETL}). 
%
\textbf{BPR} \cite{rendle2012bpr} is a representative pairwise learning-based factorization model, focusing on minimizing the ranking loss between predicted ratings and observed ratings.
%
\textbf{NeuMF} \cite{he2017neural} is a representative neural network based model, replacing the conventional inner product with a neural architecture to improve recommendation accuracy.
%
\textbf{DMF} \cite{xue2017deep} is the state-of-the-art deep neural network based recommendation model, employing a deep architecture to learn the low-dimensional factors of users and items.
%
\textbf{CoNet} \cite{hu2018conet} enables dual knowledge transfer across domains by introducing cross connections unit from one base network to the other and vice versa.
%
\textbf{DDTCDR} \cite{li2020ddtcdr} introduces a deep dual transfer network that transfers knowledge with orthogonal transformation across domains.
%
\textbf{DARec} \cite{darec19} transfers knowledge between domains with shared users, learning shared user representations across different domains via domain adaptation technique.
%
\textbf{ETL} \cite{etl} is a recent state-of-the-art CDR model that adopts equivalent transformation module to capture both the overlapped and the non-overlapped domain-specific properties.  
%
\textbf{\modelname-SYM} is a comparative model for ablation study which replaces \cdrmodel~with a symmetrical CDR framework, using auto-encoder to model both the published source rating matrix and the target rating matrix. \modelname-SYM uses JLT based differential private rating matrix publishing mechanism.
%
\textbf{\modelname-J} is our proposed \modelname~with JLT based differential private rating matrix publishing mechanism in the first stage.
%
\textbf{\modelname-S} is our proposed \modelname~with Sparse-aware JLT based differential private rating matrix publishing mechanism.

% \begin{itemize}[leftmargin=*] \setlength{\itemsep}{-\itemsep}
% \item \textbf{BPR} \cite{rendle2012bpr} is a representative pairwise learning-based factorization model, focusing on minimizing the ranking loss between predicted ratings and observed ratings.

% \item \textbf{NeuMF} \cite{he2017neural} is a representative neural network based model, replacing the conventional inner product with a neural architecture to improve recommendation accuracy.

% \item \textbf{DMF} \cite{xue2017deep} is the state-of-the-art deep neural network based recommendation model, employing a deep architecture to learn the low-dimensional factors of users and items.

% \item \textbf{CoNet} \cite{hu2018conet} enables dual knowledge transfer across domains by introducing cross connections unit from one base network to the other and vice versa.

% \item \textbf{DDTCDR} \cite{li2020ddtcdr} introduces a deep dual transfer network that transfers knowledge with orthogonal transformation across domains.

% \item \textbf{DARec} \cite{darec19} transfers knowledge between domains with shared users, learning shared user representations across different domains via domain adaptation technique.

% \item \textbf{ETL} \cite{etl} is a recent state-of-the-art CDR model that adopts equivalent transformation module to capture both the overlapped and the non-overlapped domain-specific properties.  

% \item \textbf{\modelname-SYM} is a comparative model for ablation study which replaces \cdrmodel~with a symmetrical CDR framework, using auto-encoder to model both the published source rating matrix and the target rating matrix. And it uses JLT based differential private rating matrix publishing mechanism.


% \item \textbf{\modelname-J} is our proposed \modelname~with JLT based differential private rating matrix publishing mechanism in the first stage.

% \item \textbf{\modelname-S} is our proposed \modelname~with Sparse-aware JLT based differential private rating matrix publishing mechanism.

% \end{itemize}

\nosection{Evaluation method}
To evaluate the recommendation performance, We use the leave-one-out method which is widely used in literature \cite{he2017neural}.
%
That is, we randomly reserve two items for each user, one as the validation item and the other as the test item.
%
Then, following \cite{he2017neural,hu2018conet}, we randomly sample 99 items that are not interacted by the user as the negative items. 
%
We choose three evaluation metrics, i.e., Hit Ratio (HR), Normalized Discounted Cumulative Gain (NDCG), and Mean Reciprocal Rank (MRR), where we set the cut-off of the ranked list as 5 and 10.
%

\nosection{Parameter settings}
For both source domain and target domain, we use two-layer MLP with hidden size of 500 and 200 as the network architecture and ReLU as the activation function.
%
For a fair comparison, we choose Adam \cite{kingma2014adam} as the optimizer, and tune both the parameters of \modelname~and the baseline models to their best values.
%
For differential private related parameters, we vary $\epsilon$ in $\{0.5,1.0,2.0,4.0,8.0,16.0,32.0,64.0\}$ and subspace dimension for the differential privately published rating matrix $n$ in $\{100,200,300,400,500,600,700,800\}$. 
%
For SJLT, we vary the sparsity coefficient of the reduced matrix $sp$ in $\{0.1,0.3,0.5,0.7,0.9\}$. 
%
For CDR modeling, we set batch size to 128 for both the source and target domains. 
%
The dimension of the latent embedding is set to $h = 200$. 
%
Meanwhile we set the hyper-parameter $\alpha = 100$ for user embedding alignment, since it achieves the best performance. 
%
For all the experiments, we perform five random experiments and report the average results. 
%

\subsection{Model Comparison (\textbf{RQ1} and \textbf{RQ2})}

We report the comparison results on \textbf{Douban} and \textbf{Amazon} datasets in Table \ref{tab:compare}.
%
% Note that \textbf{\modelname-J} represents \textbf{\modelname~}with JLT used in the rating publishing stage, while \textbf{\modelname-S} represents \textbf{\modelname~}with SJLT instead.
%
From the results, we can find that: (1) All the cross domain recommendations models  (e.g., \textbf{DARec}) perform better than single domain recommendation (e.g., \textbf{NeuMF}) models, indicating that cross domain recommendations can integrate more useful information to enhance the model performance, which always conform to our common sense.
%
(2) Our proposed \textbf{\modelname-J} and \textbf{\modelname-S} outperform all the single-domain and cross-domain baseline models in all tasks, which means the two-stage design of privacy-preserving CDR works well in predicting users' preference in target domain while preserving the data privacy of the source domain at the same time.
%
(3) By comparing the performance between \textbf{\modelname-J} and \textbf{\modelname-S}, we can conclude that Sparse-aware Johnson-Lindenstrauss Transform can effectively alleviate the data sparsity in the source domain, and thus significantly boosts the recommendation performance of \textbf{\modelname~}.


\begin{table*}[t]
\centering
\small
\caption{Experimental results on Amazon and Douban datasets. }
\vspace{-0.2cm}
\label{tab:compare}
\begin{tabular}{ccccccccccccc}
\toprule
\multirow{3}{*}{}
&HR@5 &NDCG@5 &MRR@5 &HR@10 &NDCG@10 &MRR@10 
&HR@5 &NDCG@5 &MRR@5 &HR@10 &NDCG@10 &MRR@10 \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
& \multicolumn{6}{c}{(Amazon) Music$\rightarrow$Book}
& \multicolumn{6}{c}{(Amazon) Movie$\rightarrow$Music}\\
% \cmidrule(lr){2-7} \cmidrule(lr){8-13}
% & \multicolumn{3}{c}{topK=5}
% & \multicolumn{3}{c}{topK=10}
% & \multicolumn{3}{c}{topK=5}
% & \multicolumn{3}{c}{topK=10}\\
% \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}

\midrule
BPR & 0.2633 & 0.2090 & 0.1827 & 0.3824 & 0.2580 & 0.2442 & 0.2448 & 0.1569 & 0.1734 & 0.3852 & 0.2035 & 0.1983 \\ 

NeuMF & 0.2760 & 0.2271 & 0.2086 & 0.4015 & 0.2577 & 0.2608 & 0.2937 & 0.1971 & 0.1988 & 0.4328 & 0.2401 & 0.2200 \\ 

DMF & 0.3075 & 0.2543 & 0.2367 & 0.4312 & 0.2713 & 0.2864 & 0.3316 & 0.2146 & 0.2266 & 0.4671 & 0.2715 & 0.2448 \\ 
\midrule 
CoNet & 0.3743 & 0.3157 & 0.3063 & 0.4831 & 0.3352 & 0.3245 & 0.3995 & 0.2857 & 0.2731 & 0.5328 & 0.3340 & 0.2973 \\ 

DDTCDR & 0.4067 & 0.3403 & 0.3241 & 0.5054 & 0.3690 & 0.3318 & 0.4311 & 0.3368 & 0.2974 & 0.5499 & 0.3736 & 0.3126 \\ 

DARec & 0.4741 & 0.3758 & 0.3420 & 0.5702 & 0.4098 & 0.3499 & 0.4916 & 0.3825 & 0.3402 & 0.6192 & 0.4220 & 0.3567 \\ 

ETL & 0.4769 & 0.3801 & 0.3462 & 0.5877 & 0.4153 & 0.3607 & 0.5308 & 0.4126 & 0.3714 & 0.6517 & 0.4511 & 0.3873 \\ 
\midrule 
\modelname-SYM & 0.4360 & 0.3467 & 0.3172 & 0.5487 & 0.3828 & 0.3321 & 0.4933 & 0.3815 & 0.3445 & 0.6103 & 0.4192 & 0.3600 \\
\modelname-J & \textbf{0.4898} & \textbf{0.3984} & \textbf{0.3648} & \textbf{0.5853} & \textbf{0.4292} & \textbf{0.3744} & \textbf{0.5399} & \textbf{0.4344} & \textbf{0.3992} & \textbf{0.6519} & \textbf{0.4706} & \textbf{0.4141} \\ 

\modelname-S & \textbf{0.5203} & \textbf{0.4264} & \textbf{0.3964} & \textbf{0.6181} & \textbf{0.4580} & \textbf{0.4092} & \textbf{0.5733} & \textbf{0.4608} & \textbf{0.4220} & \textbf{0.6853} & \textbf{0.4970} & \textbf{0.4392}  \\


\toprule

\multirow{3}{*}{}
& \multicolumn{6}{c}{(Amazon) Movie$\rightarrow$Book}
& \multicolumn{6}{c}{(Douban) Book$\rightarrow$Music}\\
% \cmidrule(lr){2-7} \cmidrule(lr){8-13}
% & \multicolumn{3}{c}{topK=5}
% & \multicolumn{3}{c}{topK=10}
% & \multicolumn{3}{c}{topK=5}
% & \multicolumn{3}{c}{topK=10}\\
% \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
% &HR@5 &NDCG@5 &MRR@5 &HR@10 &NDCG@10 &MRR@10 
% &HR@5 &NDCG@5 &MRR@5 &HR@10 &NDCG@10 &MRR@10 \\
\midrule
BPR & 0.2798 & 0.1665 & 0.2210 & 0.3716 & 0.2109 & 0.2392 & 0.1375 & 0.0822 & 0.0699 & 0.2889 & 0.1058 & 0.0950 \\ 

NeuMF & 0.3042 & 0.1989 & 0.2341 & 0.3999 & 0.2438 & 0.2403 & 0.1336 & 0.0913 & 0.0728 & 0.3042 & 0.1187 & 0.1093 \\ 

DMF & 0.3253 & 0.2281 & 0.2570 & 0.4238 & 0.2510 & 0.2439 & 0.1547 & 0.1003 & 0.0824 & 0.3315 & 0.1367 & 0.1100 \\ 
\midrule 
CoNet & 0.3744 & 0.2659 & 0.2978 & 0.4905 & 0.3050 & 0.3098 & 0.2044 & 0.1321 & 0.0996 & 0.3787 & 0.1633 & 0.1340 \\ 

DDTCDR & 0.4322 & 0.3490 & 0.3132 & 0.5288 & 0.3827 & 0.3355 & 0.2312 & 0.1425 & 0.1037 & 0.3934 & 0.1846 & 0.1506 \\ 

DARec & 0.4904 & 0.3824 & 0.3388 & 0.6034 & 0.4224 & 0.3552 & 0.2703 & 0.1878 & 0.1479 & 0.4285 & 0.2269 & 0.1711 \\ 

ETL & 0.5124 & 0.4119 & 0.3757 & 0.6339 & 0.4514 & 0.3915 & 0.3241 & 0.2161 & 0.1832 & 0.4545 & 0.2545 & 0.1987\\ 
\midrule 

\modelname-SYM & 0.4614 & 0.3665 & 0.3346 & 0.5801 & 0.4031 & 0.3496 & 0.3225 & 0.2113 & 0.1848 & 0.4535 & 0.2517 & 0.2002 \\
\modelname-J & \textbf{0.5320} & \textbf{0.4324} & \textbf{0.3992} & \textbf{0.6423} & \textbf{0.4673} & \textbf{0.4135} & \textbf{0.3290} & \textbf{0.2208} & \textbf{0.1854} & \textbf{0.4675} & \textbf{0.2643} & \textbf{0.2034} \\ 

\modelname-S & \textbf{0.5516} & \textbf{0.4483} & \textbf{0.4136} & \textbf{0.6585} & \textbf{0.4843} & \textbf{0.4285} & \textbf{0.3701} & \textbf{0.2582} & \textbf{0.2212} & \textbf{0.5097} & \textbf{0.3032} & \textbf{0.2397}  \\


\toprule

\multirow{3}{*}{}
& \multicolumn{6}{c}{(Douban) Movie$\rightarrow$Book}
& \multicolumn{6}{c}{(Douban) Movie$\rightarrow$Music}\\
% \cmidrule(lr){2-7} \cmidrule(lr){8-13}
% & \multicolumn{3}{c}{topK=5}
% & \multicolumn{3}{c}{topK=10}
% & \multicolumn{3}{c}{topK=5}
% & \multicolumn{3}{c}{topK=10}\\
% \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
% &HR@5 &NDCG@5 &MRR@5 &HR@10 &NDCG@10 &MRR@10 
% &HR@5 &NDCG@5 &MRR@5 &HR@10 &NDCG@10 &MRR@10 \\
\midrule
BPR & 0.1827 & 0.1132 & 0.1091 & 0.3436 & 0.1590 & 0.1375 & 0.1572 & 0.1079 & 0.0959 & 0.3387 & 0.1635 & 0.1134 \\ 

NeuMF & 0.1989 & 0.1279 & 0.1124 & 0.3640 & 0.1748 & 0.1453 & 0.1641 & 0.0932 & 0.0947 & 0.3462 & 0.1577 & 0.1204 \\ 

DMF & 0.2376 & 0.1438 & 0.1321 & 0.3952 & 0.1940 & 0.1511 & 0.1889 & 0.1104 & 0.1082 & 0.3754 & 0.1823 & 0.1409 \\ 
\midrule 
CoNet & 0.2736 & 0.1724 & 0.1533 & 0.4407 & 0.2330 & 0.1996 & 0.2284 & 0.1358 & 0.1305 & 0.4193 & 0.2179 & 0.1748 \\ 

DDTCDR & 0.2984 & 0.1803 & 0.1776 & 0.4699 & 0.2487 & 0.2174 & 0.2457 & 0.1639 & 0.1522 & 0.4298 & 0.2375 & 0.1846 \\ 

DARec & 0.3331 & 0.2285 & 0.2109 & 0.4970 & 0.2789 & 0.2310 & 0.2990 & 0.2017 & 0.1835 & 0.4576 & 0.2608 & 0.2081 \\ 

ETL & 0.3850 & 0.2705 & 0.2348 & 0.5247 & 0.3157 & 0.2572 & 0.3383 & 0.2357 & 0.2008 & 0.4739 & 0.2862 & 0.2286 \\ 
\midrule 
\modelname-SYM & 0.3742 & 0.2642 & 0.2310 & 0.5159 & 0.3094 & 0.2490 & 0.3194 & 0.2242 & 0.1930 & 0.4720 & 0.2737 & 0.2122 \\
\modelname-J & \textbf{0.3926} & \textbf{0.2788} & \textbf{0.2421} & \textbf{0.5349} & \textbf{0.3248} & \textbf{0.2603} & \textbf{0.3450} & \textbf{0.2496} & \textbf{0.2197} & \textbf{0.4872} & \textbf{0.2922} & \textbf{0.2373} \\ 

\modelname-S & \textbf{0.4301} & \textbf{0.3090} & \textbf{0.2702} & \textbf{0.5686} & \textbf{0.3503} & \textbf{0.2872} & \textbf{0.3801} & \textbf{0.2736} & \textbf{0.2440} & \textbf{0.5109} & \textbf{0.3158} & \textbf{0.2609}  \\
\bottomrule

\end{tabular}
%}
\end{table*}

\subsection{In-depth Model Analysis}

\nosection{Ablation study (\textbf{RQ3})}
To study whether our model is effective for the heterogeneous user-item rating data, we compare \textbf{\modelname-J} and \textbf{\modelname-S} with \textbf{\modelname-SYM}. %which replaces the \cdrmodel with a symmetrical CDR framework using auto-encoder to model both the published source rating matrix and the target rating matrix. \sjj{whether necessary to repeat the definition}
% 
The results from Table \ref{tab:compare} show that both \textbf{\modelname-J}and \textbf{\modelname-S} outperform \textbf{\modelname-SYM} in all tasks, indicating that the heterogeneous CDR model we proposed in stage two makes it easier to handle the heterogeneity of rating data produced by stage one, and thus achieves a superior performance. 
%


\nosection{Parameter analysis (\textbf{RQ4})}
We now study the effects of hyper-parameters on model performance. The most important parameters in \textbf{\modelname-J} are the privacy parameter $\epsilon$ and subspace dimension $n$.
%
The key parameter in \textbf{\modelname-S} is $sp$, which denotes the sparsity degree of the  sparse Johnson-Lindenstrauss matrix. 
%
We report the results in Fig.~\ref{fig1:param}-Fig.~\ref{fig1:param-sp}, where we use \textbf{(Amazon) Music $\rightarrow$ Book} and \textbf{(Douban) Movie $\rightarrow$ Book} datasets.
%
Fig.~\ref{fig1:param} shows the effect of $\epsilon$. %, where we vary $\epsilon$ in $\{0.5,1.0,2.0,4.0,8.0,16.0,32.0,64.0\}$. 
%
With user-level differential privacy, the published rating matrix changes with subspace dimension $n_1'$. For details, please refer to Appendix~\ref{sec:rating_dp_append}.
%
We can find that the performance gradually improves when $\epsilon$ increases and finally keeps a stable level after $\epsilon$ reaches 32.0 in \textbf{(Amazon) Music $\rightarrow$ Book}. And for the dataset \textbf{(Douban) Movie $\rightarrow$ Book}, the turning point is when $\epsilon=2.0$.
%
We also vary $n$ %in $\{100,200,300,400,500,600,700,800\}$ 
and report the results in Fig.~\ref{fig1:param-n}. The bell-shaped curve indicates that the accuracy will first gradually increase with $n$ and then slightly decrease, and \textbf{\modelname-J} achieves the best performance when $n=400$ in \textbf{(Amazon) Music $\rightarrow$ Book} and when $n=500$ in \textbf{(Douban) Movie $\rightarrow$ Book}.
%
Fig.~\ref{fig1:param-sp} shows the effect of $sp$. %, where we set $sp$ in $\{0.1,0.3,0.5,0.7,0.9\}$. 
%
The results show that when $sp$ is small (e.g., 0.1), SJLT fails to grasp enough knowledge from the rating matrix in source domain. 
%
When $sp$ is large (e.g., 0.9), SJLT gets redundant information from source domain rating matrix. 
%
A medium $sp$, e.g., 0.5 on \textbf{(Amazon) Music $\rightarrow$ Book} and 0.7on \textbf{(Douban) Movie $\rightarrow$ Book}, enables SJLT to grasp enough knowledge from the source domain rating matrix while exert an implicit regularization on optimization, and thus can achieve the best performance. 
%
% We observe that the performance peaks at $sp = 0.5$ in \textbf{(Amazon) Music $\rightarrow$ Book} and at $sp = 0.7 $ in \textbf{(Douban) Movie $\rightarrow$ Book} from Fig.~\ref{fig1:param-sp}. 
%\sjj{how to analyze the effect of $sp$}.


\begin{figure} 
    \centering
        \subfigure[Amazon Music $\rightarrow$ Book]{
    \begin{minipage}[t]{0.47\linewidth} %0.23为minipage的宽度，可以调节子图间的距离
    \includegraphics[width=4.2cm]{figures/1.pdf}
    \end{minipage}
}
        \subfigure[Douban Movie $\rightarrow$ Book]{
    \begin{minipage}[t]{0.47\linewidth} %0.23为minipage的宽度，可以调节子图间的距离
    \includegraphics[width=4.2cm]{figures/2.pdf}
    \end{minipage}
}
\vspace{-0.5cm}
	  \caption{Effect of the privacy parameter $\epsilon$ on \modelname-J. }
	  \vspace{-0.1cm}
	  \label{fig1:param}
% \vspace{-0.2cm}
\end{figure}



\begin{figure} 
    \centering
        \subfigure[Amazon Music $\rightarrow$ Book]{
    \begin{minipage}[t]{0.47\linewidth} %0.23为minipage的宽度，可以调节子图间的距离
    \includegraphics[width=4.2cm]{figures/3.pdf}
    \end{minipage}
}
        \subfigure[Douban Movie $\rightarrow$ Book]{
    \begin{minipage}[t]{0.47\linewidth} %0.23为minipage的宽度，可以调节子图间的距离
    \includegraphics[width=4.2cm]{figures/4.pdf}
    \end{minipage}
}
\vspace{-0.5cm}
	  \caption{Effect of subspace dimension $n$ on \modelname-J.}
% 	  \vspace{-0.2cm}
	  \label{fig1:param-n}
\vspace{-0.1cm}
\end{figure}


\begin{figure} 
    \centering
        \subfigure[Amazon Music $\rightarrow$ Book]{
    \begin{minipage}[t]{0.47\linewidth} %0.23为minipage的宽度，可以调节子图间的距离
    \includegraphics[width=4.2cm]{figures/5.pdf}
    \end{minipage}
}
        \subfigure[Douban Movie $\rightarrow$ Book]{
    \begin{minipage}[t]{0.47\linewidth} %0.23为minipage的宽度，可以调节子图间的距离
    \includegraphics[width=4.2cm]{figures/6.pdf}
    \end{minipage}
}
\vspace{-0.5cm}
	  \caption{Effect of sparsity param $sp$ on \modelname-S.  } 
% 	  \vspace{-0.2cm}
	  \label{fig1:param-sp}
\vspace{-0.1cm}
\end{figure}



\begin{figure} 
    \centering
        \subfigure[Amazon Movie $\rightarrow$ Music]{
    \begin{minipage}[t]{0.47\linewidth} %0.23为minipage的宽度，可以调节子图间的距离
    \includegraphics[width=4.2cm]{figures/7.pdf}
    \end{minipage}
}
        \subfigure[Douban Movie $\rightarrow$ Book]{
    \begin{minipage}[t]{0.47\linewidth} %0.23为minipage的宽度，可以调节子图间的距离
    \includegraphics[width=4.2cm]{figures/8.pdf}
    \end{minipage}
}
\vspace{-0.5cm}
	  \caption{Effect of the source domain sparsity degree $sd$. %on \modelname-J and \modelname-S.
	  }
	  \label{fig1:param-sd}
\vspace{-0.1cm}
\end{figure}

% \begin{table}[!t]
% \small
% \centering
% \caption{The results on xxx, where we set the cut-off to 5. }
% \label{tab:param}
% \begin{tabular}{cccccccc}
% \toprule
% \multirow{2}{*}{Model} & \multirow{2}{*}{$SP_{s}$}
% & \multicolumn{3}{c}{(Amazon) Movie$\rightarrow$Music}
% & \multicolumn{3}{c}{(Douban) Movie$\rightarrow$Book}\\
% \cmidrule(lr){3-5} \cmidrule(lr){6-8}
% & &HR &NDCG &MRR &HR &NDCG &MRR\\

% \midrule
% % DeepCoNN & 1.8775 & 1.8692 & 1.7434 & 1.8267\\ 
% % ESCOFILT & 1.4326 & 1.4089.& 1.3581 & 1.4033\\
% \multirow{4}{*}{\modelname-J} & 1 & 0.5399 & 0.4344 & 0.3992 & 0.3926 & 0.2788 & 0.2421\\
%  & 1/2 & 0.5366 & 0.4302 & 0.3969 & 0.3874 & 0.2731 & 0.2390\\
%  & 1/4 & 0.5302 & 0.4257 & 0.3978 & 0.3839 & 0.2690 & 0.2367\\
%  & 1/8 & 0.5280 & 0.4219 & 0.3963 & 0.3811 & 0.2665 & 0.2343\\
% \midrule 
% \multirow{4}{*}{\modelname-S} & 1 & 0.5733 & 0.4608 & 0.4220 & 0.4301 & 0.3090 & 0.2702\\
%  & 1/2 & 0.5717 & 0.4586 & 0.4200 & 0.4286 & 0.3063 & 0.2689\\
%  & 1/4 & 0.5709 & 0.4573 & 0.4207 & 0.4274 & 0.3055 & 0.2690\\
%  & 1/8 & 0.5690 & 0.4575 & 0.4210 & 0.4252 & 0.3037 & 0.2676\\
% \midrule

% \end{tabular}
% %}
% \end{table}



\nosection{Effect of source domain sparsity (\textbf{RQ5})}
To study the effect of source domain sparsity on the performance of JLT and SJLT, we change the sparsity of the source domain by sampling from the original dataset, 
%
such that the sparsity degree $sd$ could be adjusted to $\{1,1/2,1/4,1/8\}$. Here, $sd=1$ denotes the original dataset without sampling.
%
We report the results in Fig.~\ref{fig1:param-sd}, where we use \textbf{(Amazon) Movie $\rightarrow$ Music} and \textbf{(Douban) Movie $\rightarrow$ Book} datasets.
%
From the results, we can conclude that:
(1) The decrease of $sp$ brings the decrease of the performance for both JLT and SJLT.
%
(2) SJLT shows greater stability than JLT when the source domain becomes more sparse, which is owning to its sparse-aware ability, as we have analyzed in Sec.~\ref{sec:utility_ana}.



==> Privacy-Preserving CDR/sections/intro.tex <==
\section{Introduction}
\label{sec:intro}

Cross-Domain Recommendation (CDR) has been popularly studied recently, due to its powerful ability to solve the data sparsity issue of traditional recommender systems \cite{zhu2021cross}. 
%
Most existing CDR models focus on leveraging different kinds of data across multiple domains to improve the recommendation performance of a target domain (or domains) through `bridges'.  % \cite{zhu2020graphical}. 
%
Here, the data are usually users' private data, e.g., user-item rating, review, and user profile. 
%
The `bridge' refers to the linked objects between different domains such as common user, common item, and common features. 

% \begin{figure}
% \centering
% \includegraphics[width=6cm]{figures/cdr-framework.pdf}
% % \vskip -0.05in
% \caption{A general CDR framework. }
% \label{fig:cdr}
% % \vskip -0.05in
% \end{figure}

\nosection{Privacy issues in CDR}
Existing CDR models assume information can directly `transfer across the bridge', ignoring the privacy issues. 
%
% A general CDR model is shown in Figure \ref{fig:cdr}, and its key 
The key of CDR model is designing transfer strategies across bridges, e.g., cross network \cite{hu2018conet} and dual  transfer network \cite{li2020ddtcdr}. 
% mapping matrix strategy \cite{zhu2018deep}, feature combination strategy \cite{zhu2019dtcdr}, and \ccc{xxx strategy}. 
%
The above models assume all data are plaintext to both domains, which is inconsistent with reality. 
%
Since these data for CDR models usually involve user sensitive information and cannot be shared with others due to regulation reasons. 
%
Therefore, how to build CDR models on the basis of protecting data privacy becomes an urgent research problem. 
 
\nosection{Problem definition}
In this paper, we consider a two-domain cross recommendation problem for simplification. 
%
Specifically, we assume there are two domains (a source domain and a target domain) which have the same user set but different user-item interaction pairs. 
%
We also assume the user-item interactions only have rating data and leave other side-information as future work. 
%
The problem of privacy-preserving CDR is to improve the recommendation performance of the target domain by leveraging the data of the source domain, while protecting the data privacy of both domains.

\nosection{Existing work}
The existing privacy-preserving recommendation models are mainly designed for two categories, i.e., individual customers and business partners. 
%
The former assumes that each client only contains the private data of a single user \cite{nikolaenko2013privacy,hua2015dp,chen2018private}, and the existing work on this either assumes the existence of a semi-honest server or reveals middle information (e.g., latent factors) during model training. 
%
The later assumes that each client (domain) has the private data of a batch of users \cite{ogunseyi2021privacy,gao2019privacy,gao2019cross,chen2019secure,cui2021exploiting}, which can be seen as privacy-preserving CDR models. % and the existing work on this is either designed for secure social recommendation \cite{chen2019secure} or location recommendation \cite{gao2019privacy} and thus are not suitable to our problem. 
%
%There are also several research on privacy-preserving CDR so far \cite{ogunseyi2021privacy,gao2019privacy,gao2019cross,chen2019secure}. %
However, they are customized to certain settings, e.g., social recommendation \cite{chen2019secure} and  location recommendation \cite{gao2019privacy}, and thus are not suitable to our problem. 

%\nosection{Motivation}
%The proposed privacy-preserving CDR should have two abilities, i.e., \textit{security} and \textit{efficiency}, so as to be applied into practice. 
%%
%First, security is the foundation of privacy-preserving machine learning. 
%%
%Any privacy-preserving machine learning models, including recommendation models, that cannot quantity the information leakage may cause serious security concerns. 
%%
%Thus, the proposed privacy-preserving CDR model should have provable security, or at least should quantity its security. 
%%
%Second, recommender systems are usually built on large-scale datasets, and therefore, efficiency determines whether the proposed privacy-preserving CDR model can be applied in real-world applications. 

\nosection{Our proposal}
%
In this paper, we propose a novel two stage based privacy-preserving CDR framework (\modelname). 
%
In \textit{stage one}, the source domain privately publishes its user-item ratings to the target domain. %, using a novel differentially private graph publishing method. 
%
In \textit{stage two}, the target domain builds a CDR model based on its raw data and the published data of the source domain. 


\textit{Design goals.} 
The two stages in \modelname~should have the following goals. 
%
First, for stage one, user-item rating matrix publishing should not only preserve the data privacy of the source domain, but also facilitate the following CDR task. 
%
Specifically, there should be the following requirements in rating publishing. 
%
(1) \textit{Privacy-preserving.} From the published user-item ratings, the target domain should not identify whether a user has rated an item. 
%
% (2) \textit{Distance-invariant.} 
(2) \textit{Restricted isometry property.}
The nature of most recommender systems is collaborative filtering. That is, users who have similar ratings tend to share similar tastes. 
%
% Thus, compared with the original rating matrix, the published rating matrix should be distance-invariant for the same user, so that users can still \textit{collaborate} with each other. 
Thus, the published rating matrix should approximate the original one well, as the restricted isometry property stated
in the literature of matrix completion~\cite{candes2005decoding}. Thus, the users can still \textit{collaborate} with each other. 
%
(3) \textit{Sparse-awareness.} Data sparsity is a long-standing problem in recommender systems. 
%
Thus, rating publishing should be able to handle the sparse user-item rating data. 
%
%Second, for stage two, 
After rating publishing in stage one, the user-item rating data becomes heterogeneous in stage two. %, as shown in Figure \ref{fig:example}. 
%
However, most existing CDR frameworks, e.g., \cite{zhu2019dtcdr,etl,darec19,li2020ddtcdr,hu2018conet}, are symmetrical. 
%
Thus, a new CDR framework that can handle such heterogeneous data is needed. 


% The proposed privacy-preserving CDR should provide two guarantees, i.e., \textit{privacy guarantee} and \textit{utility guarantees}. 
% %
% First, privacy is the essential issue of privacy-preserving machine learning. 
% %
% Any privacy-preserving machine learning models, including recommendation models that cannot quantity the information leakage, may cause serious security concerns. 
% %
% Differential privacy ~\cite{dwork2008differential} is rigorous mathematics definition to measure privacy loss during ML training~\cite{abadi2016deep,bu2019deep}.
% % 
% Second, we build recommender systems on large-scale datasets, and therefore, utility determines whether one can apply the proposed privacy-preserving CDR model in real-world applications. 
% %
% Thus, we provide differential private version CDR under a modest privacy budget with an acceptable cost of computational complexity, training efficiency, and model quality. 

% \begin{figure}[t]
%  \begin{center}
%  \subfigure[The original rating matrix]{
%  		\label{fig:example:orig}
%  		\includegraphics[height=2.2cm]{figures/example-original.pdf}}~~
%  \subfigure[The published rating matrix]{
%  		\label{fig:example:publ}
%  		\includegraphics[height=2.2cm]{figures/example-published.pdf}}
%  	\vspace{-0.15in}
%  \caption{Example of the user-item rating publishing stage of the source domain.}
%  \vspace{-0.15in}
%  \label{fig:example}
%  \end{center}
% \end{figure}


\textit{Technical solution.} 
In stage one, inspired by the fact that Johnson-Lindenstrauss Transform (JLT) preserves differential privacy \cite{blocki2012johnson}, we propose two methods to publish rating matrix differential privately. 
%
We first propose JLT based differential private rating matrix publishing mechanism, which can not only protect data privacy but also preserve the similarity between users. %distance between users. 
%
We then propose Sparse-aware JLT (SJLT) which can further reduce the computation complexity of JLT and alleviate the data sparsity in the source domain with sub-Gaussian random matrix and Hadamard transform. 
%
We finally theoretically analyze their privacy and utility. 
%
In stage two, we propose a novel heterogeneous CDR model (\cdrmodel), which uses deep auto-encoder and deep neural network to model the published source rating matrix and target rating matrix, respectively. 
%
We also propose an embedding alignment module to align the user embeddings learnt from two networks. 

\nosection{Contributions}
% In this paper, we propose a novel differential private CDR model by adopting careful designed random transforms preserving privacy and utility.
We summarize our main contributions as follows: 
(1) We propose \modelname, a general privacy-preserving CDR framework, which has two stages, i.e., rating publishing and cross-domain recommendation modeling. 
(2) We propose two differential private rating publishing algorithms, via JLT and SJLT respectively, we also provide their privacy and utility guarantees. 
(3) We propose \cdrmodel~to handle the heterogeneous rating data between the published source domain and target domain. 
(4) We conduct experiments on two benchmark datasets and the results demonstrate the effectiveness of \modelname~and \cdrmodel.
% \begin{itemize}[leftmargin=*] \setlength{\itemsep}{-\itemsep}
% \item We propose \modelname, a general privacy-preserving CDR framework, which has two stages, i.e., rating publishing and cross-domain recommendation modeling. 
% \item We propose two differential private rating publishing algorithms, via JLT and SJLT respectively, we also provide their privacy and utility guarantees. 
% \item We propose \cdrmodel~to heterogeneous rating data between the published source domain and target domain, and propose an embedding alignment module so that information can transfer across two domains. 
% \item We conduct experiments on three benchmark datasets and the results demonstrate the effectiveness of our proposed \modelname~and \cdrmodel.
% \end{itemize}

==> Privacy-Preserving CDR/sections/model.tex <==
\section{The Proposed Framework}
\label{sec:model}

In this section, we first describe the notations and then present the framework of \modelname~and its two stages. 

% In this section, we first present the notations used throughout this paper. We then give an overview of our proposed privacy-preserving CDR algorithm ~\modelname. Thirdly, we go through the details of differential private rating matrix publishing algorithms. Finally, we present~\cdrmodel. 

\subsection{Notations}
\label{sec:model:notation}
We assume there are only two domains, i.e., domain $\mathcal{A}$ and domain $\mathcal{B}$, which have the same batch of users but different user-item pairs. 
%
We assume domain $\mathcal{A}$ has a private rating matrix $\mathbf{R}^A \in\mathbb{R}^{m\times n_1}$, and domain $\mathcal{B}$ holds another private rating matrix $\mathbf{R}^B \in\mathbb{R}^{m\times n_2}$, where $m$ denotes the number of users, $n_1$ and $n_2$ denote the number of items on domain $\mathcal{A}$ and domain $\mathcal{B}$, respectively. 
%
% We denote the user latent factor matrix as $\textbf{U}\in\mathbb{R}^{k\times m}$ and 
We use $\mathbf{U}_i^A$ and $\mathbf{U}_i^B$ to denote the latent embedding of the user $i$ on the published source domain and target domain, respectively. 
%
We also use $\mathbf{V}_j^B$ to denote the latent embedding of item $j$ on the target domain. 
% We denote the item latent factor matrix on domain $\mathcal{A}$ and domain $\mathcal{B}$ as $\textbf{V}_A\in\mathbb{R}^{k\times n_1}$ and $\textbf{V}_B\in\mathbb{R}^{k\times n_2}$, where $k$ is the dimension of latent factors. 
%
% Besides, we define two indicator matrices $\mathbf{I}^A\in\mathbb{R}^{m\times n_1}$ and $\mathbf{I}^B\in\mathbb{R}^{m\times n_2}$, where $I_{i,j}$ denotes whether user $i$ has rated item $j$ on each domain. 
%
Notice that for a matrix $\mathbf{X}$, we denote its $i$-th column as $\mathbf{x}_{i}$.
%
We summarize the main notations in Appendix~\ref{sec:app:note}. 


% \subsection{Motivation}
% As we have described in Section \ref{sec:intro}, privacy-preserving CDR requires both `privacy' and `efficiency' so that it can be applied into practice. 
% %
% First, `privacy' means that there should not be any information leakage during model training, including the user-item ratings that directly show user privacy and user-item latent factors that implicitly reflect user privacy. 
% %
% Therefore, rating, user latent factors, and item latent factors should all be kept securely for security concern during model training. 
% %
% Second, `efficiency' refers to that the proposed model should have good (\ccc{maybe linear}) scalability, which means that the proposed model should be able to handle data sparsity problem. 

% In the following of this section, we will first propose \modelone, which aims to solve the privacy issue of CDR. We will then propose \modeltwo, which improves \modelone~and solves its efficiency issue. 

\begin{figure}[t]
 \begin{center}
 \includegraphics[width=\columnwidth]{figures/framework.jpg}
 \vspace{-0.2 in}
 \caption{Framework of \modelname.}
 \vspace{-0.15 in}
 \label{fig:framework}
 \end{center}
\end{figure}

\subsection{Overview of \modelname}
We propose \modelname, a general privacy-preserving CDR framework. 
%
Similar as most existing CDR models, \modelname~aims to transfer the knowledge learnt from the source domain to help improve the recommendation performance of the target domain. 
%
However, different from the existing CDR models that assume the data from both the source and target domains are available, \modelname~aims to build a CDR model on the basis of protecting the data of both domains.  
%

\modelname~consists of two stages, i.e., \textit{rating publishing} and \textit{cross-domain recommendation modeling}, as is shown in Figure \ref{fig:framework}.
%
First, as described in Section \ref{sec:intro}, rating publishing mainly has three goals, i.e., \textbf{G1}: \textit{privacy-preserving}, \textbf{G2}: \textit{restricted isometry property}, and \textbf{G3}: \textit{sparse-aware}. 
%
To achieve these goals, we propose two differential private rating matrix publishing algorithms, including JLT and SJLT. 
%
The former one achieves \textit{privacy-preserving} and \textit{restricted isometry property} while the later one further achieves \textit{sparse-aware}, which will be further demonstrated both in theoretically in Sec.~\ref{sec:ana} and experimentally in Sec.~\ref{sec:experi}. 
%
Second, to handle the heterogeneity between the published rating matrix of the source domain and the original rating matrix of the target domain, we propose a new cross-domain recommendation model (i.e., \cdrmodel). 
%
~\cdrmodel~has three parts, a \textit{rating reconstruction module} for the published source domain, a \textit{rating regression module} for the target domain, and a \textit{user embedding alignment module} between the user embeddings of the source domain and target domain. 

With our proposed two stages, \modelname~can not only protect rating privacy, but also take advantage of the characteristics of both domains. 
%
Thus, \modelname~can achieve comparable even better performance than most existing plaintext CDR models, as will be reported in Sec.~\ref{sec:experi}. 
%
We will present these two stages in details. 

\begin{algorithm}[t]
\caption{Differential Private Rating Matrix Publishing }\label{alg:dp_rating_pub}
\KwIn{ A rating matrix $\mathbf{R}$; 
parameters: $\epsilon, \delta, \eta, \mu > 0, q = O(\frac{1}{m}) \in (0,1)$; 
number of users $m$;
number of items in the source domain: $n_1$ }
\KwOut{ Privacy preserving rating matrix $\mathbf{\tilde{R}}$ }

{
\# \textbf{Perturb the singular values of normalized $\mathbf{R}$} \\\label{alg:dp_rating_pub:begin}
Subtract the mean from $\mathbf{R}$ by computing 
%$\mathbf{R} \leftarrow \mathbf{R} - \frac{1}{m} \mathbf{1} \mathbf{1}^{\intercal} \mathbf{R};$
$r_{ij} \rightarrow r_{ij} - \frac{1}{m}\sum_{k=1}^m r_{ik};$
\\ \label{alg:dp_rating_pub:submean}
Compute $n'_1 = {8 \ln(2/\mu)}/{(\eta^2)}$ and $w = \sqrt{32 n'_1 \ln(2/\delta)}/{\epsilon} \ln(4 n'_1 /\delta);$\\
Compute the SVD of $\mathbf{R} = \mathbf{U \Sigma V^{\intercal}}$; \\
% \# \textbf{Standardize rating matrix} \\
% \# \textbf{Perturb singular values} \\
Set $\mathbf{R} \leftarrow \mathbf{U} \sqrt{\mathbf{\Sigma}^2 + w^2 \mathbf{I}} \mathbf{V}^{\intercal},$ with $\mathbf{I}$ a identity matrix. \\ \label{alg:dp_rating_pub:perfinal}
\# \textbf{Generate random matrix \textbf{M} by JLT}\\ \label{alg:dp_rating_pub:tranbegin}
Draw i.i.d. samples from $\GN(0,1)$, and form a matrix $\textbf{M} \in\mathbb{R}^{n'_1 \times n_1}$; \\
\# \textbf{Generate random matrix \textbf{M} by SJLT}\\
Generate a sparse Johnson-Lindenstrauss matrix $\mathbf{P}$ of size $n'_1 \times n_1$ using Equation \eqref{eq:def-p} \\
% ,  with 
% $$
% \mathbf{P}_{ij} \leftarrow
% \begin{cases}
% 0 \quad & \text{with probability }\quad 1-q; \\
% \xi \sim \GN(0, q^{-1}) \quad & \text{with probability }\quad q.
% \end{cases}
% $$ \\
Generate a normalized Hadamard matrix of size $n_1 \times n_1$ with 
$
\mathbf{H}_{ij} \leftarrow {n_1}^{-1/2} (-1)^{(i-1, j-1)},
$
where $(i, j) = \sum_k i_k j_k \mod 2$ is the bit-wise inner product of index $i, j$; \\
% where $(i, j)$ is the dot-product of index $i, j$ expressed in binary. \\
Generate a diagonal matrix of size $n_1 \times n_1$ using Equation \eqref{eq:def-d}\\
% with 
% $$
% \mathbf{D}_{ii}
% \leftarrow
% \begin{cases}
% -1 \quad & \text{with probability }\quad 1/2; \\
% 1 \quad & \text{with probability }\quad 1/2.
% \end{cases}
% $$ \\
Compute \textbf{M} by $\textbf{M} = \mathbf{PHD}$ \\
\# \textbf{For both JLT and SJLT} \\
Transform rating matrix $\mathbf{\tilde{R}} \leftarrow \frac{1}{\sqrt{n'_1}} \mathbf{M R};$ \\ \label{alg:dp_rating_pub:tranend}
%Compute perturbed Laplacian matrix  $\tilde{L} = \frac{1}{r} E^{\intercal} (PHD)^{\intercal} PHD E $;\\
\textbf{return} The perturbed matrix $\mathbf{\tilde{R}}$. \\
}
\end{algorithm} 

\subsection{Differential Private Rating Publishing}

We first present the rating publish stage of \modelname. 
%
We protect the source domain data by publishing the source domain rating matrix to the target domain utilizing differential privacy.
%
To protect the individual user-item rating privacy, we want the rating publishing stage to satisfy $(\epsilon, \delta)-$differential privacy. 
%
For this purpose, we propose to publish the rating matrix in the source domain differential privately via JLT or SJLT, as is shown in Algorithm~\ref{alg:dp_rating_pub}. 
%
The whole process of the rating publish stage can be divided into two procedures, i.e., \textit{perturb the singular values of the normalized rating matrix} (lines \ref{alg:dp_rating_pub:begin}-\ref{alg:dp_rating_pub:perfinal}) and \textit{transform the perturbed rating matrix by JLT or SJLT} (lines \ref{alg:dp_rating_pub:tranbegin}-\ref{alg:dp_rating_pub:tranend}). 
%
We now describe these procedures in details. 

%
% \ccc{revise according to algo 1}
% In Algorithm~\ref{alg:dp_graph}, the first step is to compute compressed dimension $r$ and re-weight parameter $w \in (0, m)$, 
% with $m$ denoting the number of users. 
\nosection{Explanation of hyper-parameters}
First of all, we introduce the hyper-parameters used Algorithm~\ref{alg:dp_rating_pub}. $\epsilon$ and $\delta$ are privacy-related hyper-parameters. We tune $\epsilon$ for different privacy budget and fix $\delta=1/n$, where $n$ is number of input data. 
$\mu$ and $\eta$ are utility-related hyper-parameters to determine the subspace dimension $n_1'$ after applying JLT or SJLT. The larger $\mu$ and $\eta$, the smaller $n_1'$, the smaller probability we get for the concentration results in Theorem~\ref{thm:RIP}. 

\nosection{Perturb the singular values of the normalized rating matrix}
Before applying random transforms on rating matrix, we apply singular value perturbation, which consists of four steps. 
% 
The first step is to subtract the mean from rating matrix $\mathbf{R}$ (line \ref{alg:dp_rating_pub:submean}).
%
The second step is to compute the compressed dimension $n_1'$ and singular value perturbation $w$ (line 3). 
%
% The second step is to re-weight input rating matrix $\mathbf{R}$ with weight $\frac{w}{m}$.
%
% The third step is to generate a Gaussian orthogonal random matrix of size $r \times d$, where $r$ is the compressed dimension and $d = n_1$ is the number of items in source domain. 
The third step is to compute the singular value decomposition of matrix $\mathbf{R}$ and get the singular values as the non-zero elements of the diagonal matrix $\Sigma$ (line 4). 
% 
The fourth step is to modify the singular values of $\mathbf{R}$ by $\sqrt{\sigma_i^2 + w^2}$, where $\sigma_i = \Sigma_{ii}$ (line 5). 
%
By exerting proper singular value perturbation on the randomized rating matrix, we get a perturbed rating matrix with the same singular vectors but a different spectrum from the original rating matrix. 
%
In recommender systems, it is common to use the singular vectors corresponding to top singular values. 
%
Thus, we preserve the privacy by perturbing the singular values while maintaining utility by keeping singular vectors unchanged, which achieves \textbf{G1}: \textit{privacy-preserving}. 

\nosection{Transform the perturbed rating matrix by JLT or SJLT} 
After the first procedure, one can transform the perturbed rating matrix randomly via JLT (line 7 and line 14) or SJLT (line 9-12 and line 14). 
%whose main difference is how to generate the random matrix $\mathbf{M}$. 
%
By applying random transform, we exert a proper randomness on rating matrix where the magnitude is determined by perturbation parameter $w$ in the previous procedure. 
%
By the expectation approximation result (Proposition~\ref{prop:mean_approx}) and 
concentration result of Gaussian or sub-Gaussian random matrix ( Proposition~\ref{prop:jl}), we conclude that JLT and SJLT achieve \textbf{G2:} \textit{restricted isometry property} ( see Theorem~\ref{thm:RIP}). 
%
The main difference between JLT and SJLT is how to generate the random matrix $\mathbf{M}$.
%
The random matrix $\mathbf{M}$ of JLT is generated by Gaussian ensemble, while that of SJLT is generated by sub-Gaussian ensemble and random Hadamard matrix, as described in Definition~\ref{def:fjlt}. 
%
By singular value perturbation and random transform with JLT or SJLT, we get a differentially privately published rating matrix $\mathbf{\tilde{R}}$. 
%
Compared with JLT, 
%
(1) SJLT can reduce the computation complexity of matrix multiplication by utilizing random Hardmard transform with computation complexity of $O(d \log d m)$ while JLT costs $O(d n m)$ (line 14).
%
(2) the random hardmard transform $\mathbf{HD}$ in SJLT serves as a precondition when input $x$ is sparse (verified by Lemma~\ref{lem:rhd}), %and the non-zeros are too rare to ensure a sufficiently strong measure concentration, which will be verified by Lemma~\ref{lem:rhd}, 
and thus SJLT achieves \textbf{G3:} \textit{sparse-awareness}. 

%
% We present the differential private rating matrix publishing algorithm via SJLT in Algorithm~\ref{alg:dp_graph2}. 
% %
% The only difference between Algorithm~\ref{alg:dp_graph2} and Algorithm~\ref{alg:dp_graph} is the generation of random matrix. 
% %
% The random matrix $\mathbf{M}$ in Algorithm~\ref{alg:dp_graph} is generated by Gaussian ensemble, where the random matrix $\mathbf{PHD}$ in Algorithm~\ref{alg:dp_graph2} is generated by Sparse-aware JLT defined in Definition~\ref{def:fjlt}. 

% The last step is perturb the rating matrix $\mathbf{R}$ by the random matrix $M$ and get a differentially privately published rating matrix $\mathbf{\tilde{R}}$. 

% Second, to enable the successive cross-domain model training, the rating publishing stage should be distance-invariant. 
% \huiwen{not exactly distance-invariant but retain the distance in a small error with a large distance.} 
% %
% That is, compared with the original rating matrix, one may expect the differential private publishing rating matrix has a distance-invariant property for the same users, 
% %the published rating matrix should be distance-invariant for the same user, 
% so that users can still \textit{collaborate} with each other. 
% %
% To this end, we utilize the concentration result of random transform ( Theorem~\ref{thm:con_jlt}).  
% %and ~\ref{thm:con_fjlt}. %
% Suppose $\mathbf{x} = \mathbf{u} - \mathbf{v}$ is the distance between two rating vectors in rating matrix $\mathbf{R}$. By Theorem~\ref{thm:con_jlt}, we see the distance between the two rating vectors $\| \mathbf{x} \| = \| \mathbf{u} - \mathbf{v}\|$ is bounded by $\left( d (1-\eta), d(1 + \eta)\right)$ with a large probability $1 - \exp(-\eta^2 d/8)$. 
% %
% Thus the correlations between users are preserved to a certain extent with a large probability.


% To conclude, by decomposing rating matrices and transforming with random matrices, we achieve \textbf{G2} which is highly related to the utility of \modelname. 
% %
% By perturbing the singular values, we achieve \textbf{G1}, and by improving JLT to SJLT, we achieve \textbf{G3}. 
% %
% We will further analyze the privacy and utility of our proposed rating publishing stage in Sec.~\ref{sec:ana}. 



%To enable the successive cross-domain model training, the rating publishing stage should have distance-preserving property.  

% In Sec.~\ref{sec:utility_ana}, we will analyze our model utility via the concentration results of JLT and SJLT. 
% %
% Compared with the original rating matrix, one may expect the differential private publishing rating matrix preserves distance in a tiny neighbor with a significant probability for the same users. Thus the users can still \textit{collaborate} with each other. 
% %
% Theoretically, we will illustrate this property via the concentration result of random transform ( Theorem~\ref{thm:con_concen}).  
% Suppose $\mathbf{x} = \mathbf{u} - \mathbf{v}$ is the distance between two rating vectors in rating matrix $\mathbf{R}$. By Theorem~\ref{thm:con_jlt}, we see the distance between the two rating vectors $\| \mathbf{x} \| = \| \mathbf{u} - \mathbf{v}\|$ is bounded by $\left( d (1-\eta), d(1 + \eta)\right)$ with a large probability $1 - \exp(-\eta^2 d/8)$. 
% %
% Thus according to the utility analysis, we preserve the similarity between users in a small neighborhood with a large probability. We explan more details in Sec.~\ref{sec:utility_ana}. 



% DP Publishing GCN via JL transform 
% \begin{algorithm}[t]
% \caption{Differential Private Rating Matrix Publishing Mechanism}\label{alg:dp_graph}
% \textbf{Input}: A rating matrix $\mathbf{R}$; 
% parameters: $\epsilon, \delta, \eta, \mu > 0$;
% number of users: $m$;
% number of items in the source domain: $n_1$\\
% \textbf{Output}: Privacy preserving rating matrix $\mathbf{\tilde{R}}$

% \begin{algorithmic}[1] %[1] enables line numbers
% \STATE Compute $n'_1 = {8 \ln(2/\mu)}/{(\eta^2)}, $ and $w = \sqrt{32 n'_1 \ln(2/\delta)}/{\epsilon} \ln(4 n'_1 /\delta);$
% \STATE For every $i \neq j$, set $r_{ij} \leftarrow \frac{w}{m} + (1 - \frac{w}{m}) r_{ij};$
% \STATE Draw i.i.d. samples from $\GN(0,1)$, and form a matrix $\textbf{M} \in\mathbb{R}^{n'_1 \times n_1}$ ;
% %where $d = n$; 
% \STATE Compute perturbed rating matrix $\mathbf{\tilde{R}}\leftarrow \mathbf{M} \mathbf{R}$;
% %Compute perturbed Laplacian matrix  $\tilde{L} = \frac{1}{r} E^{\intercal} M^{\intercal} M E $;\\
% %Compute perturbed degree matrix $\tilde{D}_{ii} = \sum_{j} (\tilde{L}_{ij}) ; $
% \STATE \textbf{return} The perturbed rating matrix $\mathbf{\tilde{R}}$.
% \end{algorithmic}
% \end{algorithm} 


% \begin{algorithm}[t]
% \caption{Differential Private Rating Matrix Publishing Mechanism}\label{alg:dp_graph}
% \KwIn{A rating matrix $\mathbf{R}$; parameters: $\epsilon, \delta, \eta, \mu > 0$; number of users: $m$; number of items in the source domain: $n_1$}
% \KwOut{Privacy preserving rating matrix $\mathbf{\tilde{R}}$}
% {
% Compute $n'_1 = {8 \ln(2/\mu)}/{(\eta^2)}, $ and $w = \sqrt{32 n'_1 \ln(2/\delta)}/{\epsilon} \ln(4 n'_1 /\delta);$\\
% Subtract the mean from $\mathbf{R}$ by computing 
% $\mathbf{R} \leftarrow \mathbf{R} -  \frac{1}{m} \mathbf{1} \mathbf{1}^{\intercal} \mathbf{R};$ \\
% Compute the SVD of $\mathbf{R} = U \Sigma V^{\intercal}$; \\
% Set $\mathbf{R} \leftarrow U \sqrt{\Sigma^2 + w^2 I_{m \times n_1'}} V^{\intercal};$ \\ 
% %For every $i \neq j$, set $r_{ij} \leftarrow \frac{w}{m} + (1 - \frac{w}{m}) r_{ij};$\\
% Draw i.i.d. samples from $\GN(0,1)$, and form a matrix $\textbf{M} \in\mathbb{R}^{n'_1 \times n_1}$; \\
% Compute perturbed rating matrix $\mathbf{\tilde{R}}\leftarrow \frac{1}{\sqrt{n'_1}} \mathbf{M} \mathbf{R}$; \\
% %Compute perturbed Laplacian matrix  $\tilde{L} = \frac{1}{r} E^{\intercal} M^{\intercal} M E $;\\
% %Compute perturbed degree matrix $\tilde{D}_{ii} = \sum_{j} (\tilde{L}_{ij}) ; $
% } 
% \textbf{return} A perturbed matrix $\mathbf{\tilde{R}}$. \\
% \end{algorithm} 

% DP Publishing GCN via Fast JL transform 


% DP Publishing GCN via Fast JL transform 
% \begin{algorithm}[t]
% \caption{Differential Private Sparse Rating Matrix Publishing Mechanism }\label{alg:dp_graph2}
% \textbf{Input}: A rating matrix $R$; 
% parameters: $\epsilon, \delta, \eta, \mu > 0, q = O(\frac{1}{m}) \in (0,1)$; 
% number of users $m$;
% number of items in the source domain: $n_1$ \\
% \textbf{Output}: Privacy preserving rating matrix $\mathbf{\tilde{R}}$

% \begin{algorithmic}[1] %[1] enables line numbers
% \STATE Compute $n'_1 \leftarrow  \frac{8 \ln(2/\mu)}{\eta^2}, $ and $w \leftarrow \sqrt{32 n'_1 \ln(2/\delta)}/{\epsilon} \ln(4 n'_1 /\delta);$
% \STATE For every $i \neq j$, set $r_{ij} \leftarrow \frac{w}{m} + (1 - \frac{w}{m}) r_{ij};$
% \STATE Generate a sparse Johnson-Lindenstrauss matrix $P$ of size $n'_1 \times n_1$,  with 
% $$
% \mathbf{P}_{ij} \leftarrow
% \begin{cases}
% 0 \quad & \text{with probability }\quad 1-q; \\
% \xi \sim \GN(0, q^{-1}) \quad & \text{with probability }\quad q.
% \end{cases}
% $$
% \STATE Generate a normalized Hadamard matrix of size $n_1 \times n_1$ with 
% $$
% \mathbf{H}_{ij} \leftarrow {n_1}^{-1/2} (-1)^{(i-1, j-1)},
% $$
% where $(i, j)$ is the dot-product of index $i, j$ expressed in binary. 
% \STATE Generate a diagonal matrix of size $n_1 \times n_1$ with 
% $$
% \mathbf{D}_{ii}
% \leftarrow
% \begin{cases}
% -1 \quad & \text{with probability }\quad 1/2; \\
% 1 \quad & \text{with probability }\quad 1/2.
% \end{cases}
% $$
% \STATE Compute perturbed rating matrix $\mathbf{\tilde{R}} \leftarrow \mathbf{PHD R};$ 
% %Compute perturbed Laplacian matrix  $\tilde{L} = \frac{1}{r} E^{\intercal} (PHD)^{\intercal} PHD E $;\\
% \STATE \textbf{return} A perturbed matrix $\mathbf{\tilde{R}}$.
% \end{algorithmic}
% \end{algorithm} 

% With Algorithm~\ref{alg:dp_graph} and Algorithm~\ref{alg:dp_graph2}, we obtain differential private published rating matrix $\mathbf{R}$.
% %
% After the rating publishing stage, the rating matrix of the source domain turns from a high-dimensional sparse matrix to a relative low-dimensional dense matrix. 
% %
% We will analyze the privacy and utility of Algorithm~\ref{alg:dp_graph} and Algorithm~\ref{alg:dp_graph2} %over rating matrix $R$ and approximation property of perturbed $\tilde{R}$ 
% in Section~\ref{sec:ana}.

% The following algorithm presents the approach to approximating $\Phi_G(S)$. 

% \begin{algorithm}[t]
% \caption{Approximating $\Phi_G(S)$}\label{alg:phi_approx}
% \KwIn{A non empty $S \subset V(G)$, parameters $n, w$ and Laplacian $\tilde{L}$ from Algorithm~\ref{alg:dp_graph}.}
% \KwOut{$R(S) = \frac{1}{1 - \frac{w}{n}} \left( \mathbf{1}_S^{\intercal} \tilde{L} \mathbf{1}_S - w \frac{s(n - s)}{n} \right)$}
% \end{algorithm}


\subsection{CDR Modeling}

We then present the cross-domain modeling stage of \modelname. 
%
The cross-domain modeling stage is done by the target domain by using the published rating matrix of the source domain and the original rating matrix of the target domain. 
%


We propose a novel cross-domain recommendation model, i.e., \cdrmodel, to solve the heterogeneity between the published rating matrix of the source domain and the original rating matrix of the target domain. 
%
\cdrmodel~has three parts: (1) a rating reconstruction module for the differential privately published source domain; (2) a rating regression module for the target domain; and (3) a user embedding alignment module between the user embeddings of the source domain and target domain. 
%
We will describe these three modules separately in detail. 

\nosection{Rating reconstruction of the source domain}
Let $\mathbf{R}^A \in\mathbb{R}^{m\times n_1}$ be the private rating matrix of the source domain, $\textbf{R}'^A \in\mathbb{R}^{m\times n'_1}$ be the published rating matrix of the source domain, and $n'_1 < n_1$. 
%
Considering that $\mathbf{R}'^A$ is a dense matrix with each row denoting the perturbed behaviors of each user, we use auto-encoder to learn user embedding. 
%
Specifically, we can first obtain the user embedding by the encoder, i.e., $\mathbf{U}_i^A=E(\mathbf{R}'^A_i) \in\mathbb{R}^{m\times h}$, where $h$ is the dimension of user embedding. 
%
The autoencoder can then reconstruct the perturbed ratings of each user by $\hat{\mathbf{R}'}^A_i = D(\mathbf{U}_i^A) \in\mathbb{R}^{m\times n'_1}$.
%
After it, the reconstruction loss is given by:
\begin{equation}
\begin{aligned}
\label{equ:recon}
\mathcal{L}_{rec} = \sum_{i=1}^m  \mathcal{F}(\mathbf{R}'^A_i, \hat{\mathbf{R}'}^A_i) ,
\end{aligned}
\end{equation}
where $\mathcal{F}(\cdot,\cdot)$ is the mean square loss.
%
With the rating reconstruction module, the encoder and decoder can model the perturbed user-item rating interactions in the source domain. 

\nosection{Rating regression of the target domain}
The rating regression module in the target domain is similar as the existing deep neural network based recommendation models, e.g., Deep Matrix Factorization (DMF) \cite{xue2017deep} and Neural Matrix Factorization (NeuMF) \cite{he2017neural}. 
%
In this paper, we take DMF as an example. 
%
The key idea of DMF is to minimize the cross-entropy between the true ratings $\textbf{R}^B_{ij}$ and the predicted ratings $\hat{\mathbf{R}}^B_{ij}$, where the predicted ratings is obtained by multiple fully-connected layers. 
%
Specifically, we first get the user and item latent embeddings $\mathbf{U}_i^B \in\mathbb{R}^{m\times h}$ and $\mathbf{V}_j^B \in\mathbb{R}^{n^2 \times h}$ with $h$ denoting the embedding dimension, and then the predicted ratings are the cosine similarities between user and item latent embeddings, i.e., $\hat{\mathbf{R}}^B_{ij} = (\mathbf{U}_i^B)^T \mathbf{V}_j^B$. 
%
Its loss function is given as:
\begin{equation}
% \tiny
\begin{aligned}
\mathcal{L}_{reg} = \sum_{i=1}^m \sum_{j=1}^{n_2} \left(
 \frac{\mathbf{R}^B_{ij}}{\max(\mathbf{R}^B)} log (\hat{\mathbf{R}}^B_{ij}) + (1-\frac{\mathbf{R}^B_{ij}}{\max(\mathbf{R}^B)}) log (1 - \hat{\mathbf{R}}^B_{ij})) \right) ,
\end{aligned}
\end{equation}
where $\max(\mathbf{R}^B)$ is the maximum rating in the target domain.
%
With the rating regression module, we can model the user-item rating interactions in the target domain.

\nosection{User embedding alignment between source and target domains}
Although the rating reconstruction module and the rating regression module can model the perturbed ratings of the source domain and the original ratings of the target domain respectively, the knowledge learnt from the source domain cannot be transferred to the target domain yet. 
%
To facilitate the knowledge transfer between the source and target domains, we further propose a user embedding alignment module. 
%
The user embedding alignment module aims to match the user embedding learnt from the rating reconstruction module and the user embedding learnt from the rating regression module. 
% 
Our motivation is that users tend to have similar preferences across different domains. 
%
For example, users who like romantic movies are likely to like romantic book as well. 
%
Formally, the user embedding alignment loss is given as:
\begin{equation}
\begin{aligned}
\mathcal{L}_{ali} = \sum_{i=1}^m {\|\mathbf{U}_i^A - \mathbf{U}_i^B\|}^2 . 
\end{aligned}
\end{equation}

\nosection{Total loss}
The loss of \cdrmodel~is a combination of the three type of losses above. That is, 
\begin{equation}
\begin{aligned}
\mathcal{L} = \mathcal{L}_{rec} + \mathcal{L}_{reg} + \alpha \mathcal{L}_{ali},
\end{aligned}
\end{equation}
where $\alpha$ is a hyper-parameter that controls the strength of the user embedding alignment module. 

% \nosection{Model training}


==> Privacy-Preserving CDR/sections/preliminary.tex <==
\section{Preliminaries}
\label{sec:pre}

% In this section, we present some preliminary techniques on constructing random transformations for rating publishing. 

\subsection{User-item Rating Differential Privacy}
%
Differential privacy is a robust, meaningful, and mathematically rigorous definition of privacy~\cite{dwork2014algorithmic}. 
%
The goal of differential privacy is to learn information about the population as a whole while protecting the privacy of each individual~\cite{dwork2011firm, dwork2007ad}. 
%
By a careful design mechanism, differential privacy controls the fundamental quantity of information that can be revealed with changing one single individual ~\cite{jiang2016wishart}.
%% Basic intro of DP 
Before diving into the differential private mechanism for user-item rating matrix publishing, we first introduce some basic knowledge on differential privacy. 

% % neighbor datasets 
% \begin{definition}~\label{def:neigh_data}(Neighbouring Datasets)
% Two datasets $S$ and $S'$ are neighbouring if exactly one element in $S$ is changed arbitrarily to obtain $S'$. 
% Formally, suppose $S = \{s_1, \cdots, s_n\}$ and $S' = \{ s'_1, \cdots, s'_n \}$, there exists $0 < j \leq n$ such that 
% $$
% \begin{cases}
% s_i \neq s_i',  \quad & i = j; \\
% s_i = s_i',  \quad & i \neq j. 
% \end{cases}
% $$
% \end{definition}

% general DP 

% \begin{definition}\label{def:dp} (Differential Privacy \cite{dwork2014algorithmic}). 
% A randomized algorithm $\M$ that takes as input a dataset consisting of individuals is $(\epsilon, \delta)-$differentially private (DP) if for any pair of datasets $S, S'$ that differ in the record of a single individual, and any event $E$, 
% \begin{equation}
% P [\mathcal{M}(x) \in E ] \leq \exp(\epsilon) P[\mathcal{M}(y) \in E] + \delta, 
% \end{equation}
%  If $\delta = 0$, we say that $\mathcal{M}$ is $\epsilon-$differentially private. 
% \end{definition}

In the scenario of recommender systems, we have a rating matrix $\mathbf{R}$ as defined in Definition~\ref{def:uirate}. 
%
Under such setting, we also define the neighbouring rating matrices in Definition~\ref{def:neigh_rating}. 
%

% rating matrix 
\begin{definition}[User-item Rating Matrix]
Let $\mathbf{U} = \{\mathbf{u}_1, \cdots, \mathbf{u}_m \}$ be a set of users
and $\mathbf{V} = \{\mathbf{v}_1, \cdots, \mathbf{v}_n \}$ be a set of items. 
Define user-item rating matrix $\mathbf{R} = \begin{bmatrix} r_{ij} \end{bmatrix}$ with $r_{ij} \geq 0$ denoting the rating of user $i$ on item $j$. 
\label{def:uirate}
\end{definition}

% \nosection{User-level Neighbouring Rating Matrices}

% neighbor rating matrix 
% \begin{definition}[User-level Neighbouring Rating Matrices]
% %\cite{zamani2020learning}
% Tow rating matrices $\mathbf{R}$ and $\mathbf{R}'$ are neighbouring if exactly one user-item rating for a certain user in $\mathbf{R}$ is changed arbitrarily to obtain $\mathbf{R}'$. 
% Suppose $\mathbf{R} = \begin{bmatrix} r_{ij} \end{bmatrix}_{n \times m}$ and $\mathbf{R}' = \begin{bmatrix} r_{ij}' \end{bmatrix}_{n \times m}$, there exists one pair $(i_0, j_0)$ with $1< i_0 < n$ and $1 < j_0 < m$ such that 
% $$
% \begin{cases}
% r_{ij} \neq r_{ij}',  \quad & i = i_0, \quad j = j_0; \\
% r_{ij} = r_{ij}',  \quad & i = i_0, \quad j \neq j_0. 
% \end{cases}
% $$
% ~\label{def:neigh_user_rating}
% \end{definition}

% \nosection{Rating-level Neighbouring Rating Matrices}

% neighbor rating matrix 
\begin{definition}[Neighbouring Rating Matrices]
%\cite{zamani2020learning}
Two rating matrices $\mathbf{R}$ and $\mathbf{R}'$ are neighbouring if exactly one user-item rating in $\mathbf{R}$ is changed arbitrarily to obtain $\mathbf{R}'$. 
Suppose $\mathbf{R} = \begin{bmatrix} r_{ij} \end{bmatrix}_{n \times m}$ and $\mathbf{R}' = \begin{bmatrix} r_{ij}' \end{bmatrix}_{n \times m}$, there exists one pair $(i_0, j_0)$ with $1< i_0 < n$ and $1 < j_0 < m$ such that 
$$
\begin{cases}
r_{ij} \neq r_{ij}'\quad \text{and} \quad |r_{ij} - r_{ij}'| <1,  \quad & i = i_0, \quad j = j_0; \\
r_{ij} = r_{ij}',  \quad & i \neq i_0, \quad j \neq j_0. 
\end{cases}
$$
~\label{def:neigh_rating}
\end{definition}
%
% Similarly, by reducing Definition~\ref{def:neigh_rating}, we have neighbouring user-item vectors, see Appendix~\ref{append:neigh_user_item}. 

% privacy loss 
To measure the privacy leakage of a randomized algorithm $\M$, we define the privacy loss on neighbouring rating matrices below. %(Definition~\ref{def:neigh_rating}). 

\begin{definition}[Privacy Loss~\cite{dwork2014algorithmic}]
Let $\mathbf{R}$ and $\mathbf{R}'$ be two neighbouring rating matrices, %defined in Definition~\ref{def:neigh_rating}, 
%
$\M$ be a randomized algorithm, $\M(\mathbf{R})$ and $\M(\mathbf{R}')$ be the probability distributions induced by $\M$ on $\mathbf{R}$ and $\mathbf{R}'$ respectively. 
%
The privacy loss is a random variable defined as 
$$
\mathcal{L}_M^{\mathbf{R},\mathbf{R}'}(\theta)\doteq\log(P(\mathcal{M}(\mathbf{R})=\theta)/P(\mathcal{M}({\mathbf{R}'})
=\theta).
$$
where $\theta \sim \M(\mathbf{R})$,
\label{def:privacy_loss}
\end{definition}



We want to protect the privacy of each user-item rating pair ($r_{ij}$), i.e., by changing a single $r_{ij}$ such that the output result of $\M$ is almost indistinguishable. 
%
% That is, we want to protect the privacy of each user-item rating pair. 
%
Thus, we define the differential privacy with respect to user-item rating matrix $\mathbf{R}$ in Definition~\ref{def:rating_dp}.

\begin{definition}[User-level Differential Privacy] 
A randomized algorithm $\M$ that takes a user-item vector as input is $(\epsilon, \delta)-$differential private if for any differ-by-one user-item vectors $\mathbf{v}, \mathbf{v}'$, and any event $\mathcal{A}$, 
\begin{equation}
P [\mathcal{M}(\mathbf{v}) \in \mathcal{A} ] \leq \exp(\epsilon) P[\mathcal{M}(\mathbf{v}') \in \mathcal{A}] + \delta. 
\end{equation}
 If $\delta = 0$, we say that $\M$ is $\epsilon-$differentially private. \label{def:user_rating_dp}
\end{definition}

\begin{definition}[Rating Matrix Differential Privacy]
A randomized algorithm $\M$ that takes rating matrix $\mathbf{R}$ as input guarantees $(\epsilon, \delta)-$differential privacy (DP) if for any pair of neighbouring rating matrices $\mathbf{R}, \mathbf{R}'$, and any event $\mathcal{A}$, 
\begin{equation}
P [\mathcal{M}(\mathbf{R}) \in \mathcal{A} ] \leq \exp(\epsilon) P[\mathcal{M}(\mathbf{R}') \in \mathcal{A}] + \delta. 
\end{equation}
 If $\delta = 0$, we say that $\M$ is $\epsilon-$differentially private. \label{def:rating_dp}
\end{definition}

% To evaluate the utility of the random transformations, we further propose the matrix approximation property based on graph approximation property~\cite{blocki2012johnson}. 


% In CDR setting, to achieve the distance-invariant property, we also define the matrix approximation property, based on graph approximation property~\cite{blocki2012johnson}. 
% \huiwen{no explicit use of matrix approximation def.}


% %%Matrix Approximation
% \begin{definition}[Matrix Approximation]
% Define an algorithm $\M$ gives $(\eta, \tau, \nu)-$approximation for matrix $\mathbf{R}$ such that the following condition holds. 
% For nonempty set $S$ and for all $s \in S$, with probability greater or equal than $1 - \nu$, we have that 
% $$
% [(1 - \eta)  \mathbf{R}^{\intercal} \mathbf{R} - \tau \leq \M(\mathbf{R})^{\intercal} \M(\mathbf{R}) \leq (1 + \eta) \mathbf{R}^{\intercal} \mathbf{R}  + \tau ]. 
% $$
% \end{definition}


\subsection{Random Transform}
We present two random transforms which preserve DP. 
% \ccc{citation in the following two definitions?} fix. 

%% JL transform 

\begin{definition}[Johnson-Lindenstrauss Transform (JLT)~\cite{blocki2012johnson}]
The Johnson-Lindenstrauss that transforms a vector $\x$ from $\mathbb{R}^d$ to $\mathbb{R}^{d'}$ is defined by $\Phi: \x \rightarrow \mathbf{M} \x$, where $\mathbf{M} \sim \GN(0, \mathbf{O}_{d' \times d})$, where $\mathbf{O}_{d' \times d}$ is a dense matrix with all elements equal one. 
\label{def:jlt}
\end{definition}


%% FAST JL transform 
% Johnson-Lindenstrauss transform (JLT) is a random projection of $m$ points from a $n-$dimensional space to a lower dimensional space such that the $\ell_2-$norm of transformed vector is maintained with a large probability.
Sparse-aware JLT performs similarly as JLT, which maps a high-dimensional space to a lower-dimensional space with $\ell_2-$norm of transformed vector maintained with a significant probability. 

\begin{definition}[Sparse-aware JLT (SJLT)~\cite{ailon2009fast}]
The SJLT that transforms a sparse vector from $\mathbb{R}^d$ to $\mathbb{R}^{d'}$ is defined by $\Psi: \x \rightarrow \mathbf{M} \x$, where $\mathbf{M} = \mathbf{P H D}$ with $\mathbf{P} \in \mathbb{R}^{d' \times d}$, $\mathbf{H} \in \mathbb{R}^{d \times d}$, $\mathbf{D} \in \mathbb{R}^{d \times d}$
% $$
% \Psi: \x \rightarrow \mathbf{M} \x, \mathbf{M} = \mathbf{P H D}, \text{with}~ \mathbf{P} \in \mathbb{R}^{d' \times d}, \mathbf{H} \in \mathbb{R}^{d \times d}, \text{and}~ \mathbf{D} \in \mathbb{R}^{d \times d}, 
% $$
\begin{equation}\label{eq:def-p}
\mathbf{P}_{ij} = 
\begin{cases}
0 \quad & \text{with probability }\quad 1-q; \\
\xi \sim \GN(0, q^{-1}) \quad & \text{with probability }\quad q;
\end{cases}
\end{equation}
$
\mathbf{H}_{ij} = d^{-1/2} (-1)^{(i-1, j-1)}
$
is the normalized Hadamard matrix where $(i, j) = \sum_k i_k j_k \mod 2$ is the bit-wise inner product mod 2, and $\mathbf{D}$ is a random diagonal matrix where 
%$\mathbf{D}_{ii} = \pm 1$ with equal probability. 
\begin{equation}\label{eq:def-d}
\mathbf{D}_{ii} = \pm 1 \quad \text{with equal probability.}
% \mathbf{D}_{ii}
% = 
% \begin{cases}
% -1 \quad & \text{with probability }\quad 1/2; \\
% 1 \quad & \text{with probability }\quad 1/2.
% \end{cases}
\end{equation}

% \begin{itemize}
% \item 
% %$P \in \mathbb{R}^{r \times d}$, $d = {n \choose 2}$ 
% $
% \mathbf{P}_{ij} = 
% \begin{cases}
% 0 \quad & \text{with probability }\quad 1-q; \\
% \xi \sim \GN(0, q^{-1}) \quad & \text{with probability }\quad q;
% \end{cases}
% $\\
% \item 
% %$H \in \mathbb{R}^{d \times d}$ 
% $
% \mathbf{H}_{ij} = d^{-1/2} (-1)^{(i-1, j-1)},
% $
% is the normalized Hadamard matrix, where $(i, j) = \sum_k i_k j_k \mod 2$ is the bit-wise inner product mod 2;\\
% \item 
% %$D \in \mathbb{R}^{d \times d}$ 
% $
% \mathbf{D}_{ii}
% = 
% \begin{cases}
% -1 \quad & \text{with probability }\quad 1/2; \\
% 1 \quad & \text{with probability }\quad 1/2.
% \end{cases}
% $\\
% \end{itemize}
\label{def:fjlt}
\end{definition}



==> Privacy-Preserving CDR/sections/relatedwork.tex <==
\section{Related Work}
\label{sec:rw}
% In this section, we briefly review the literature on cross domain recommendation and privacy-preserving recommendation. 

\subsection{Cross Domain Recommendation}
Cross Domain Recommendation (CDR) is proposed to
handle the cold-start and data sparsity problem commonly existed in the traditional single domain recommender systems \cite{zhu2021cross}. 
%
The basic assumption of CDR is that different behavioral patterns from multiple domains jointly characterize
the way users interact with items \cite{pan21dual,zhu2019dtcdr}. 
%
Thus, CDR models can improve the recommendation performance of the single domain recommender systems by transferring the knowledge learnt from other domains using auxiliary information. 
%
To date, different kinds of knowledge transferring strategies are proposed in CDR, e.g.,  cross
connections \cite{hu2018conet}, dual learning \cite{li2020ddtcdr}, and adversarial training \cite{darec19}. 
%
However, most existing CDR models assume information can directly `transfer across the bridge', ignoring the privacy issues. 
%
In this paper, we aim to solve the privacy issue in CDR using differential privacy. 

\subsection{Privacy-Preserving Recommendation}

Most existing privacy-preserving recommendation models are built to protect the data privacy of individual customers (2C) rather than business partners (2B). 
%
The main difference between  these two types of models is the data distribution on clients. 
%
The former (2C case) assumes that each client only contains the private data of a single user, while the later (2B case) assumes that each client has the private data of a batch of users. 
%
The representative work of the 2C models include 
\cite{mcsherry2009differentially,ziqidpmf,nikolaenko2013privacy,hua2015dp,chen2018private}, which use different types of techniques. 
%
For example, McSherry et al.~\cite{mcsherry2009differentially} presented a differential private recommendation method by adding plain Gaussian noise on the covariance matrix. 
%
% Nikolaenko et al. \cite{nikolaenko2013privacy} applied garbled circuits for secure matrix factorization, and it has high security but low efficiency. 
%
Hua et al. \cite{hua2015dp} adopted differential privacy for matrix factorization, and there is a trade-off between privacy and accuracy. 
%
Chen et al. \cite{chen2018private} proposed decentralized matrix factorization and can only applied for point-of-interest recommendation. 
%
% Chai et al. \cite{chai2020secure} incorporated homomorphic encryption for federated matrix factorization.
% , but it has two shortcomings. 
% %
% First, a server is needed to aggregate item latent factors, and it assumes the server is semi-honest and not collude with clients, which may not exist in practice. 
% %
% Second, item latent factors are revealed to clients, which is not provable secure and may cause privacy leakage, since item latent factors are learnt using the clients' user latent factors.  
%
The representative work of the 2B model includes \cite{chen2019secure,gao2019privacy,liu2021fedct,ogunseyi2021privacy,cui2021exploiting}. 
%
First, the model in \cite{chen2019secure} was designed for secure social recommendation, which is not suitable to the situations where all the domains have user-item rating data. 
%
Second, \cite{gao2019privacy} was designed for location recommendation, which uses differential privacy to protect user location privacy and is not suitable to our problem. 
% using transfer learning technique, which is not provable secure and does not suitable to our problem. 
Besides, \cite{ogunseyi2021privacy} uses somewhat homomorphic encryption and thus %can only scale
is limited to only small-scale dataset (with hundreds of users). 

In summary, the existing privacy-preserving recommendation approaches are either designed for 2C scenario or 2B scenarios that are not suitable to our problem. 
%
In this paper, we propose to adopt differential privacy for 2B scenario where two domains have the same batch of users but different sets of items. 

% \subsection{Differential Privacy}


% \subsection{Random Transform}
% Researchers discover random linear and nonlinear random transformations that project high-dimensional vectors into low-dimensional subspace to preserve statistical information and reduce computational complexity while keeping $\ell_2-$distance of pairwise vectors with a high probability. 
% % 
% Nonlinear random transformations to a low-dimensional manifold show their benefits in some scenario~\cite{}, which we will not cover in this paper.
% %
% Researchers construct linear ones based on the nice Johnson-Lindenstrauss lemma that random transform preserves pairwise distance with a high probability. And they further improve the random transform for economical storage and fast computation.
% %
% The original construction of the Johnson-Lindenstrauss is a random matrix consisting of orthonormal vectors~\cite{johnson1984extensions}. 
% In this construction, one requires orthonormality to maximizing the mutual information from a statistical perspective. In this case, the matrix is dense and needs the orthogonalization process, heavy in storage and computation. 
% % 
% Indyk and Motwani~\cite{indyk1998approximate}, Dasgupta and Gupta~\cite{dasgupta2003elementary} propose random matrix with each entry as i.i.d. Gaussian. In this case, the orthogonalization process is redundant because random unit vectors are mutually orthogonal with large probability. 
% %
% Achilioptas~\cite{achlioptas2003database} shows that by replacing a Gaussian random variable with a sub-Gaussian random variable, we still have the Johnson-Lindenstrauss lemma with an efficient computation. Each entry in the random matrix equals $0$ with a probability of $2/3$ and $\pm 1$ with $1/6$. 
% % 
% Motivated by the Uncertainty Principle in harmonic analysis: a nonzero function and its Fourier transform cannot both be sharply localized, 
% Ailon and Liberty~\cite{ailon2009fast} propose a fast Johnson-Lindenstrauss transform by combining a fast Fourier transform and a sparse Johnson-Lindenstrauss transform to improve performance. 






==> sections/analysis.tex <==
\section{Analysis}\label{sec:ana}

In this section, we provide privacy and utility analysis of our proposed DP rating publishing algorithm (Algorithm~\ref{alg:dp_rating_pub}).  

% Privacy analysis 

%---------------------------------------------------------------------------------------------------------------------------------------------------
%
%									Privacy Analysis 						
%
%---------------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Privacy Analysis}
% In this section, we derive the privacy property of the two proposed random DP publishing algorithms, Algorithm~\ref{alg:dp_graph} and Algorithm~\ref{alg:dp_graph2}.
%
Differential Privacy~\cite{dwork2014algorithmic} is a rigorous mathematics definition to measure the difficulty for an adversary to identify the presence or absence of any individual in a data-set via leveraging the output of a random algorithm $\M$. 
%
A general way to analyze the privacy of a random algorithm $\M$ is to tail bound the privacy loss random variable, defined by the log of the division of the output distributions on neighboring data sets.  
%
Thus, to provide the privacy analysis of Algorithm~\ref{alg:dp_rating_pub}, we study how the output distribution changes by differ exactly one user-item rating $r_{ij}$ in the input rating matrix $\mathbf{R}$. 
%

We will first show the eigenvalue interlacing for rating matrix in Lemma~\ref{lem:interlace_2}. 
%
By the eigenvalue interlacing results, we will then present the upper and lower bounds for privacy loss in Lemma~\ref{lem:upper} and Lemma~\ref{lem:lower} respectively. 
%
After it, by combining with the k-fold Composition Theorem in Theorem~\ref{thm:k_fold_comp}, we will show that Algorithm~\ref{alg:dp_rating_pub} achieves $(\epsilon, \delta)$ in Theorem~\ref{thm:dp_graph}. 

\nosection{Eigenvalue interlacing for rating matrix}
%
Suppose we have two neighbouring rating matrices $\mathbf{R}$ and $\mathbf{R}'$ as defined in Definition~\ref{def:neigh_rating}. 
%
Without loss of generality, we assume a rating $r_{ij}$ is not in $\mathbf{R}$ but in $\mathbf{R'}$. 
%
With line 2 in Algorithm~\ref{alg:dp_rating_pub} performing on $\mathbf{R}$, we have that $r_{ij}$ is with the value $\frac{w}{m}$ in $\mathbf{R}$ and with the value $r_{ij} \leftarrow \frac{w}{m} + (1 - \frac{w}{m}) r_{ij}$ in $\mathbf{R}'$. 
Define the covariance matrix of $\mathbf{R}$ as 
$\mathbf{L} = \mathbf{R}^{\intercal} \mathbf{R}$. 
%
After using Algorithm~\ref{alg:dp_rating_pub},
the $(i,j)$ element in $\mathbf{L}$ becomes $l_{ij} + \left( 1 - \frac{w}{m} \right) \Delta l_{ij}$, where $\Delta l_{ij} = r_{ik}^{\intercal} r_{jk}$. 
%
Thus, we can derive the eigenvalue interlacing lemma (Lemma~\ref{lem:interlace_2}) by the eigenvalue interlacing for minors which we presented in Lemma 1 in Appendix. 

% \begin{lemma} 
% [Eigenvalue Interlacing for Minors] Let $\mathbf{A}$ be an $n \times n$ symmetric matrix with eigenvalues 
% $\lambda_1 \leq \lambda_2 \leq \cdots \lambda_n$, and $\mathbf{B}$ be any $(n-1) \times (n-1)$ principal minor sub-matrix of $\mathbf{A}$, with eigenvalues $\mu_1 \leq \mu_2 \leq \cdots \leq \mu_{n-1}.$ Then 
% $$
% \lambda_i \leq \mu_i \leq \lambda_{i+1}, \quad \forall 1 \leq i \leq n-1. 
% $$
% \label{lem:interlace_1}
% \end{lemma}

\begin{lemma} 
[Eigenvalue Interlacing for Rating Matrix]
Assume 
$ \mathbf{R}^{\intercal} = \mathbf{U \Sigma V^{\intercal}} and~ \mathbf{R'}^{\intercal} = \mathbf{ U' \Lambda V'^{\intercal}},$ with 
$\mathbf{\Sigma} = \rm{diag} \left( \begin{bmatrix} \sigma_1, \cdots, \sigma_{n-1}, \sigma_n \end{bmatrix}  \right)$ 
and 
$\mathbf{\Lambda} = \rm{diag} \left( \begin{bmatrix} \lambda_1, \cdots, \lambda_{n-1}, \lambda_n \end{bmatrix}  \right)$ 
be the singular values of~$\mathbf{R}$~and~$\mathbf{R'}$ respectively, we have   
$$
\forall i, \quad \sigma_i \leq \lambda_i \leq \sigma_{i+1}. 
$$
\label{lem:interlace_2}
\end{lemma}

\begin{proof}
\ccc{Proof. in appendix}
\end{proof}

%---------------------------------------------------------------------------------------------------------------------------------------------------
%
%						Johnson-Lindenstrauss Transform 
%
%---------------------------------------------------------------------------------------------------------------------------------------------------

\nosection{Analysis for user-level differential privacy?}
\ccc{rewrite this para.}
\nosection{Lower and upper bounds for privacy loss in one row}
%
To guarantee the privacy of Algorithm~\ref{alg:dp_graph} and Algorithm~\ref{alg:dp_graph2}, we analyze how the output distribution changes as exactly one value changes in the input rating matrix. 
% 
% We outline the proof of Algorithm~\ref{alg:dp_graph} as follows. 
%
Suppose $\mathbf{R}$ and $\mathbf{R'}$ are two neighbouring rating matrices as defined in Definition~\ref{def:neigh_rating}. 
%
As the privacy loss $L_{\M}^{\mathbf{R}, \mathbf{R'}}$ defined in Definition~\ref{def:privacy_loss}, we are interested in the difference of output distributions $\M(\mathbf{R})$ and $\M(\mathbf{R}')$. 
%
To do this, we first summarize Algorithm~\ref{alg:dp_graph} and Algorithm~\ref{alg:dp_graph2} as follows. 

\noindent\textit{Algorithm ~\ref{alg:dp_graph}.}
We summarize Algorithm~\ref{alg:dp_graph} as the following two operations on the input rating matrix $\mathbf{R}$, i.e., 
\begin{itemize}
    \item $\mathbf{R} \leftarrow \frac{w}{m}  \mathbf{I} + (1 - \frac{w}{m}) \mathbf{R}$, 
    \item $\mathbf{\tilde{R}} = \mathbf{M} \mathbf{R},$ with $\mathbf{M} \sim \GN(0, \mathbf{I}_{n_1' \times n_1})$, 
\end{itemize}
where $\mathbf{M}$ is constructed by concatenating $n'_1$ i.i.d. random Gaussian vectors $\mathbf{Y} \sim \GN(\mathbf{0}, \mathbf{I}_{n \times 1})$. 

%
In order to check the distribution between the output rating matrices $\mathbf{\tilde{R}}$ and $\mathbf{\tilde{R}'}$, we first compare the difference in Probability Density Function (PDF) of a single row in $\mathbf{\tilde{R}}$ and $\mathbf{\tilde{R}'}$, i.e., 
$\mathbf{R}^{\intercal} \mathbf{Y}$ and ${\mathbf{R}'}^{\intercal} \mathbf{Y}$.


% \huiwen{arrive the same intermediate results in Lemma 2 and Lemma 3}
\noindent\textit{Algorithm ~\ref{alg:dp_graph2}.}
Algorithm~\ref{alg:dp_graph2} is a modification of Algorithm~\ref{alg:dp_graph}. 
%
Specifically, in the step operation, the random transform is changed from a Gaussian orthogonal ensemble $\textbf{M}$ defined in Definition~\ref{def:jlt} to a sparse Johnson-Lindenstrauss transform, i.e., $\mathbf{PHD}$, defined in Definition~\ref{def:fjlt}, where $\mathbf{P}$ is a sparse Gaussian matrix, $\mathbf{H}$ is a Hadamard matrix and $\mathbf{D}$ is a random diagonal matrix. 
%
By construction, we have two good properties for Algorithm~\ref{alg:dp_graph2}. 
\begin{itemize}
    \item $\mathbf{D}$ and $\mathbf{U}$ are unitary, i.e., 
    $
    \mathbf{D}^{\intercal} \mathbf{D} = \mathbf{I}; \quad 
    \mathbf{U}^{\intercal} \mathbf{U} = \mathbf{I}, 
    $
    \item Rows in $\mathbf{P}$ are sub-Gaussian, 
\end{itemize}
%
where $\mathbf{P}$ is constructed by concatenating $n'_1$ i.i.d. sparse random Gaussian vectors $\mathbf{Y}$, where 
$$
\mathbf{Y}_i = 
\begin{cases}
0, \quad & \quad \text{with probability } 1-q; \\
\xi \sim \GN(0, q^{-1})& \quad \text{with probability } q. 
\end{cases}
$$


%
In order to check the distribution between $\mathbf{\tilde{R}}$ and $\mathbf{\tilde{R}}'$, for Algorithm~\ref{alg:dp_graph} and Algorithm~\ref{alg:dp_graph2}, we compare the difference in Probability Density Function (PDF) of a single row in $\mathbf{\tilde{R}}$ and $\mathbf{\tilde{R}'}$, i.e., 
$\mathbf{R}^{\intercal} \mathbf{Y}$ and ${\mathbf{R}'}^{\intercal} \mathbf{Y}$,  with $\mathbf{Y}$ denoting a Gaussian vector or sparse Gaussian vector.
%
%--------------------------------------------------%
%
%           User-level Differential Privacy 
%
%---------------------------------------------------%

In this section, we present the privacy loss of a single row in differential private published rating matrix $\mathbf{\tilde{R}},$ i.e., user-level differential privacy. The main result is described as follows. 

\begin{lemma}
Suppose $\mathbf{R}$ and $\mathbf{R}'$ are two neighbouring rating matrix as defined in Definition~\ref{def:neigh_rating}. 
%
$\mathbf{Y}$ is Gaussian random vectors defined before. 
%

\end{lemma}


% we focus on the privacy property by comparing the distributions $\mathbf{R}^{\intercal} \mathbf{Y}$ and $\mathbf{R}'^{\intercal} \mathbf{Y}.$ \ccc{where is $\mathbf{\tilde{R}}'$ for algo. 2?}
%
% Through previous analysis \ccc{where?}, one can explore the difference of distribution on one row of the output matrices, i.e., $\mathbf{R}^{\intercal} \mathbf{Y}$ and $\mathbf{R}'^{\intercal} \mathbf{Y}$, with $\mathbf{Y}$ denoting a Gaussian vector or sparse Gaussian vector.
%
% With the similar deduction, we arrive the same lower and upper bound of the difference between $\pdf_{\mathbf{R}^{\intercal} \mathbf{Y}}$ and $\pdf_{\mathbf{R}'^{\intercal} \mathbf{Y}}$ for Algorithm~\ref{alg:dp_graph} and Algorithm~\ref{alg:dp_graph2}, and we summarize them in Lemma~\ref{lem:lower} and Lemma~\ref{lem:upper} respectively. 

% \begin{lemma} [Lower Bound] \label{lem:lower}
% Set $\epsilon_0 = \frac{\epsilon}{\sqrt{4 n_1' \ln(2/\delta)}}$, $ \delta_0 = \frac{\delta}{2 n_1'}$, and denote $S = \{ x: \pdf_{\mathbf{R}^{\intercal} \mathbf{Y}} (x) \geq e^{-\epsilon_0}  \pdf_{\mathbf{R}^{\intercal} \mathbf{Y}} (x) \}$ with $\mathbf{Y}_{n_1 \times 1}$ a Gaussian random vector or a sparse Gaussian random vector, 
% we have
% \begin{equation} \label{eqn:lower}
% P (S) \geq 1 - \delta_0. 
% \end{equation}
% \end{lemma}

% \begin{lemma} [Upper Bound] \label{lem:upper}
% Set $\epsilon_0 = \frac{\epsilon}{\sqrt{4 n_1' \ln(2/\delta)}}$, $ \delta_0 = \frac{\delta}{2 n_1'}$, 
% %$\mathbf{Y}$ is a random vector of size $n \times 1$ with every element is a normal random variable, i.e., $\mathbf{Y} \sim \GN(\mathbf{0}, \mathbf{I}_{n \times 1})$
% with $\mathbf{Y}_{n_1 \times 1}$ a Gaussian random vector or a sparse Gaussian random vector, 
% we have
% \begin{equation}\label{eqn:upper}
% \forall x, \pdf_{\mathbf{R}^{\intercal} \mathbf{Y}} (x) \leq e^{\epsilon_0} \pdf_{{\mathbf{R}'}^{\intercal} \mathbf{Y}} (x).
% \end{equation}
% \end{lemma}


% The rating matrix and the covariance matrix shares the same spectrum property as shown in Lemma~\ref{lem:interlace_2}. It is equivalent to compare the distributions of covariance matrices $\M(\mathbf{L})$ and $\M(\mathbf{L}')$. 
% %
% Under Algorithm~\ref{alg:dp_graph}, the output covariance matrix is to 
% $\mathbf{\tilde{L}}= \frac{1}{n_1'} \mathbf{R}^{\intercal} \mathbf{M}^{\intercal} \mathbf{M} \mathbf{R} = \mathbf{O}^{\intercal} \mathbf{O}$ and 
% $\mathbf{\tilde{L}'} = \frac{1}{n_1'} \mathbf{R}'^{\intercal} \mathbf{M}^{\intercal} \mathbf{M} \mathbf{R}' = \mathbf{O}'^{\intercal} \mathbf{O}'$ respectively, 
% with $M \sim \GN(\mathbf{0}, \mathbf{I}_{d' \times n})$ a Gaussian orthogonal ensemble (GOE) as defined in Definition~\ref{def:jlt}. 
% % 
% We concate $\mathbf{O}$ by $k$ i.i.d. random vector $Y \sim \GN(\mathbf{0}, \mathbf{I}_{n \times 1})$. 
% %
% In order to check the distribution between the output covariance matrices $\mathbf{\tilde{L}}$ and $\mathbf{\tilde{L}'}$, we first compare the difference in probability density function of $\mathbf{R}{\intercal} Y$ and $\mathbf{R}^{\intercal} Y$.
%
% In the following lemma, we prove the upper bound of the difference between $\pdf_{\mathbf{R}^{\intercal} \mathbf{Y}}$ and $\pdf_{{\mathbf{R}'}^{\intercal} \mathbf{Y}}. $


% \begin{lemma} \label{lem:upper}
% Set $\epsilon_0 = \frac{\epsilon}{\sqrt{4 r \ln(2/\delta)}}, \delta_0 = \frac{\delta}{2r}.$
% $\mathbf{Y}$ is a random vector of size $n \times 1$ with every element is a normal random variable, i.e. $\mathbf{Y} \sim \GN(\mathbf{0}, \mathbf{I}_{n \times 1})$
% Then 
% \begin{equation}\label{eqn:upper}
% \forall x, \pdf_{\mathbf{R}^{\intercal} \mathbf{Y}} (x) \leq e^{\epsilon_0} \pdf_{{\mathbf{R}'}^{\intercal} \mathbf{Y}} (x).
% \end{equation}

% \end{lemma}

% Then we comes to the lower bound of the difference between two distributions $\pdf_{\mathbf{R}^{\intercal} \mathbf{Y}}$ and $\pdf_{{\mathbf{R}'}^{\intercal} \mathbf{Y}}. $


% \begin{lemma} \label{lem:lower}
% Set $\epsilon_0 = \frac{\epsilon}{\sqrt{4 r \ln(2/\delta)}}, \delta_0 = \frac{\delta}{2r}.$
% And denote $S = \{ x: \pdf_{\mathbf{R}^{\intercal}_G \mathbf{Y}} (x) \geq e^{-\epsilon_0}  \pdf_{\mathbf{R}^{\intercal}_{G'} \mathbf{Y}} (x) \}$
% \begin{equation} \label{eqn:lower}
% P (S) \geq 1 - \delta_0
% \end{equation}
% \end{lemma}



%---------------------------------------------------------------------------------------------------------------------------------------------------
%
%						Fast Johnson-Lindenstrauss Transform 
%
%---------------------------------------------------------------------------------------------------------------------------------------------------
%
% To guarantee privacy of Algorithm~\ref{alg:dp_graph2}, we are interested in the distributions of output covariance matrices
% $\mathbf{\tilde{L}}$ and $\mathbf{\tilde{L}'}$ on the two neighboring rating values $\mathbf{R}$ and $\mathbf{R}'.$
% %
% Under Algorithm~\ref{alg:dp_graph2}, the output covariance matrix is
% $\mathbf{\tilde{L}} = \frac{1}{d'} \mathbf{R}^{\intercal} (\mathbf{PHD})^{\intercal} \mathbf{PHD} \mathbf{R} = \frac{1}{d'} \mathbf{R}^{\intercal} \mathbf{P}^{\intercal} \mathbf{P} \mathbf{R}$ and 
% $\mathbf{\tilde{L}'} = \frac{1}{d'} \mathbf{R'}^{\intercal} (\mathbf{PHD})^{\intercal} \mathbf{PHD} \mathbf{R'} = \frac{1}{d'} 
% \mathbf{R'}^{\intercal} \mathbf{P}^{\intercal} \mathbf{P} \mathbf{R'}$ respectively, 
% with $\mathbf{P}$ is a sparse Gaussian matrix, $\mathbf{H}$ is a Hadamard matrix and $\mathbf{D}$ is a diagonal matrix as defined in Algorithm~\ref{alg:dp_graph2}. 
% By construction, $\mathbf{D}$ and $\mathbf{U}$ are unitary, i.e., 
% $$
% \mathbf{D}^{\intercal} \mathbf{D} = \mathbf{I}; \quad 
% \mathbf{U}^{\intercal} \mathbf{U} = \mathbf{I}. 
% $$
% %
% We construct $\mathbf{P}$ by $k$ i.i.d. sparse random Gaussian vector $\mathbf{Y}$. 
% %
% In order to check the distribution between $\mathbf{\tilde{L}}$ and $\mathbf{\tilde{L}}'$, we focus on the privacy property by comparing the distributions $\mathbf{R}^{\intercal} \mathbf{Y}$ and $\mathbf{R}'^{\intercal} Y.$
% %
% With similar deduction in previous section, we prove the upper bound of the difference between $\pdf_{\mathbf{R}^{\intercal} \mathbf{Y}}$ and $\pdf_{\mathbf{R}'^{\intercal} \mathbf{Y}}. $


% \begin{lemma} \label{lem:upper2}
% Set $\epsilon_0 = \frac{\epsilon}{\sqrt{4 r \ln(2/\delta)}}, \delta_0 = \frac{\delta}{2r}.$
% Then 
% \begin{equation}\label{eqn:upper2}
% \forall x, \pdf_{\mathbf{R}^{\intercal}_G \mathbf{Y}} (x) \leq e^{\epsilon_0} \pdf_{\mathbf{R}^{\intercal}_{G'} \mathbf{Y}} (x).
% \end{equation}
% \end{lemma}

% Then we get the lower bound of the difference between two distributions $\pdf_{\mathbf{R}^{\intercal}_G \mathbf{Y}}$ and $\pdf_{\mathbf{R}^{\intercal}_{G'} \mathbf{Y}}$. 
% \ccc{cannot follow}
% \huiwen{try to see the difference between the two distributions, pdf -- probability density function.}

% \begin{lemma} \label{lem:lower2}
% Set $\epsilon_0 = \frac{\epsilon}{\sqrt{4 r \ln(2/\delta)}}, \delta_0 = \frac{\delta}{2r}.$
% And denote $S = \{ x: \pdf_{\mathbf{R}^{\intercal}_G \mathbf{Y}} (x) \geq e^{-\epsilon_0}  \pdf_{\mathbf{R}^{\intercal}_{G'} \mathbf{Y}} (x) \}$
% \begin{equation} \label{eqn:lower2}
% P (S) \geq 1 - \delta_0
% \end{equation}
% \end{lemma}



%---------------------------------------------------------------------------------------------------------------------------------------------------
\nosection{Analysis for rating-level differential privacy?}
\ccc{rewrite this para.}
\nosection{Differential privacy rating publishing algorithms}
By previous lower and upper bounds, we compare the distribution difference of a single row in output rating matrix $\mathbf{\tilde{R}}$ and $\mathbf{\tilde{R}}'$. To analyze the difference of two whole rating matrices $\mathbf{\tilde{R}}$ and $\mathbf{\tilde{R}}'$, we utilize the following composition theorem presented in Theorem~\ref{thm:k_fold_comp}. 

\begin{theorem} [Composition Theorem \cite{dwork2010boosting}]
For every $\epsilon >0, \delta, \delta' >0$, and $k \mathbb{N},$ the class of $(\epsilon, \delta)-$differential private mechanisms is 
$(\epsilon', k \delta + \delta')-$differentially private under $k-$fold adaptive composition, for 
$
\epsilon' = \sqrt{2k \ln (1/\delta')} \epsilon + k \epsilon \epsilon_0
$,
where $\epsilon_0 = e^{\epsilon} -1.$
\label{thm:k_fold_comp}
\end{theorem}

With the privacy guarantee of one row in $\mathbf{R}$ and composition theorem, we present differential privacy with respect to rating value of Algorithm~\ref{alg:dp_graph} and Algorithm~\ref{alg:dp_graph2}.

\begin{theorem}[Rating matrix differential privacy] %\cite{blocki2012johnson}
%of Algorithm~\ref{alg:dp_graph}]
Algorithm~\ref{alg:dp_graph} and Algorithm~\ref{alg:dp_graph2} preserve $(\epsilon, \delta)-$differential privacy with respect to a single rating value changing in $\mathbf{R}$. 
\label{thm:dp_graph}
\end{theorem}

\begin{proof}
\ccc{add proof description?}
\end{proof}

%---------------------------------------------------------------------------------------------------------------------------------------------------
%
%						Utility Analysis 
%
%---------------------------------------------------------------------------------------------------------------------------------------------------

\subsection{Utility Analysis}
\label{sec:utility_ana}

In this section, we present the utility analysis of differential private rating matrix publishing mechanism, Algorithm~\ref{alg:dp_graph} and Algorithm~\ref{alg:dp_graph2} with concentration results of JLT and SJTL. 

\begin{theorem}
[Concentration of JLT~\cite{upadhyay2013random} and SJLT~\cite{ailon2009fast}]
For any $\eta \in (0, 1/2)$ and $M$ be a $n_1' \times n_1$ random matrix, as defined in Definition~\ref{def:jlt} or Definition~\ref{def:fjlt}. 
For $\forall \mathbf{x} \in \mathbb{R}^n,$ let $S =\{ \x:  (1- \eta) \| \x \|^2 \leq \frac{1}{n_1'} \| \mathbf{M} \x \|^2 \leq (1 + \eta) \| \x \|^2 \}$, we have
$$
P\left[ S \right] \geq 1- 2 \exp(- \eta^2 n_1'/8). 
$$
\label{thm:con_jlt}
\end{theorem}

% It is easy to check $\mathbf{HD}$ is $\ell_2-$norm preserving. $\mathbf{P}$ is a sparsity version of $M$, then we have the concentration results of 
% $\mathbf{PHD}$, i.e., 

% \begin{theorem}[Concentration of SJLT~\cite{ailon2009fast}]
% Suppose the same assumptions as described in Theorem~\ref{thm:con_jlt}.
% Let $\mathbf{P}, \mathbf{H}, \mathbf{D}$ be random matrices as defined in Definition~\ref{def:fjlt}. 
% Let $S = \{\x: (1- \eta) \| \x \|^2 \leq \frac{1}{n_1'} \| \mathbf{PHD} \x \|^2 \leq (1 + \eta) \| \x \|^2 \}$, we have 
% $$
% \mathbf{P} \left[ S  \right] \geq 1 -2 \exp (- \eta^2 n_1'/8). 
% $$
% \label{thm:con_fjlt}
% \end{theorem}

Following the concentration results of Johnson-Lindenstrauss (Theorem~\ref{thm:con_jlt} and Theorem~\ref{thm:con_fjlt}), 
%and the algorithm approximating $\Phi_G$ (Algorithm~\ref{alg:phi_approx}),
we have the utility guarantees of Algorithm~\ref{alg:dp_graph} and Algorithm~\ref{alg:dp_graph2}. For details of proof, please refer to ~\cite{blocki2012johnson}.
%
Furthermore, 
with random transform used in Algorithm~\ref{alg:dp_graph} and Algorithm ~\ref{alg:dp_graph2}, we have a good approximation of the original rating matrix $\mathbf{R}$ with a large probability, as is shown in Theorem~\ref{thm:dp_approx}. 


\begin{theorem}[Approximation Property~\cite{blocki2012johnson}]
For every $\eta, \mu > 0$, $\tau = O \left(s \frac{\sqrt{\ln(1/\delta) \ln(1/\mu)}}{\epsilon}  \left( \ln(1/\delta) + \ln(\ln(1/\mu)/ \eta^2) \right)\right)$, and a nonempty $S$ of size $s$, Algorithm~\ref{alg:dp_graph} and Algorithm~\ref{alg:dp_graph2} give a $(\eta, \tau, \mu)-$approximation for rating matrix $\mathbf{R}$.
~\label{thm:dp_approx}
\end{theorem}


















